Theoretical and Observational Aspecs in Metric-Affine Gravity: A field theoretic perspective

In this PhD thesis we deal with several theoretical and phenomenological apsects of metric-affine theories of gravity. Concretely, we first give a broad introduction to the necessary tools to understand the framework and elaborate on some subtleties of the minimal coupling prescription between geometry and matter in presence of torsion and nonmetricity. Then we dedicate the central part of the thesis to study the structure of Ricci Based gravity (RBG) theories, which will be of later use to understand generic properties of metric-affine theories. We begin by analysing the structure of the RBG field equations and nontrivial aspects of their solution space. We then analyse the abrosption spectra of some spherically symmetric solutions. Then, we show that, if the projective symmetry in these theories is explicitly broken, then there arise ghost degrees of freedom, and we argue that this will be a generic feature of metric-affine gravity theories. Having done this, we analyse metricafine theories through the EFT lens, showing how the nonmetricity tkes a particular form in generic theories where the symmetrised Ricci tensor appears in the action beyond the Einstein-Hilbert term. This sources effective interactions that we use to place tight constraints to these theories. In the third part of the thesis we present a miscelanea of works which are not so related to the structure of RBG theories. We begin by studying a model for spontaneous breaking of Lorentz symmetry, namely the bumblebee model, in the metric-affine approach. In the following chapter we generalise a conformal invariant definition of proper time given by Perlick to the case with general nonmetricity. Finally, we present arguments that show that the recently proposed D4EGB theory is not well defined in its original form. We finish with a brief outlook.

==> Chapters/Part03.tex <==
%
% File: chap01.tex
% Author: Victor F. Brena-Medina
% Description: Introduction chapter where the biology goes.
%
\let\textcircled=\pgftextcircled

\part{Funhouse}

\markboth{Part III}{}

{\noindent\Large\textbf{Part III - Outline}}
\vspace{0.5cm}

This is the last part of the thesis. The name is just a pun which reminds us that we do science because we have fun with it, just as The Stooges did with their music. However, this should not be interpreted as being less rigorous material. Here we develop some interesting ideas that sprouted in more relaxed environments, such as interesting conversations with friends (and collaborators, or a linear combination of both), reflections about some peculiar issues, or speculative ideas that, in one or the another way, have led to some curious and interesting results that could or could not lead to deeper insights on the properties of gravitation. Thus, in contrast with the two previous parts, the reader should expect to find a miscellanea of works which need not be in close connection to each other, but where interesting results have been achieved.

\chapter{Covariant actions for Loop Cosmologies}\label{sec:LQC}


The idea of quantising symmetry-reduced cosmological spacetimes {\it \`a la Loop} dates back to \cite{Bojowald:1999tr}, and consistent quantisation was achieved in \cite{Ashtekar:2006rx,Ashtekar:2006wn,Ashtekar:2006es}. There it was shown that the resulting isotropic and homogeneous cosmological model predicted a big bounce replacing the Big Bang singularity, a prediction which has later proven to be robust if anisotropies were allowed \cite{Ashtekar:2007em}. However, Loop quantisation of cosmological backgrounds presents ambiguities in the quantisation process regarding how the Euclidean and Lorentzain terms of the Hamiltonian constraint are treated. In recent years, different cosmological models tied to these ambiguities have been presented \cite{Agullo:2016tjh,Yang:2009fp}. Symmetry reduction makes the Lorentzian term be proportional to the Euclidean one at the classical level. In standard Loop Quantum Cosmology (LQC), the quantisation is carried out after the Lorentzian term is written in terms of the Euclidean one. However, quantisation ambiguities arise due to the possibility of treating both constraints independently in the quantisation process, leading to different effective Hamiltonians which are expected to be closer in spirit to full Loop Quantum Gravity (LQG). Concretely, two such Hamiltonians that have already been studied are those governing mLQC-I and mLQC-II \cite{Li:2018fco}. In both cases the Big Bang singularity is replaced by a bounce at around Planckian curvatures. While mLQC-II predicts a symmetric bounce just as standard LQC, consistent dynamics for mLQC-I requires an asymmetric bounce with a prebounce branch that is asymptotically de Sitter in the past \cite{Li:2018opr}. 

Following the spirit of the work by Olmo and Singh \cite{Olmo:2008nf}, our aim here is to find a covariant action that provides an effective classical description of the background evolution in mLQC-I and mLQC-II. As we will see, indeed, there is a family of covariant metric-affine $f(R)$ theories that can encode the background evolution of the post-bounce branches\footnote{Note that the post- and pre- bounce branches are identical in LQC and mLQC-II, so that in those cases the effective description covers the full cosmological evolution.} of mLQC-I and mLQC-II, as well as that of standard LQC with a choice of parameters. As a cross-check,  will see how for the choice of parameters that lead to standard LQC the corresponding classical effective action recovers the result found in \cite{Olmo:2008nf}.

\section{Background evolution equivalence}

The background evolution of a cosmological model in metric-affine $f(R)$ theories can be derived from the RBG field equations\footnote{Note that metric-affine $f(R)$ theories are a subset of RBG theories.} \eqref{eq:MetricFieldEquationsRBGEinsteinForm}, which assuming homogeneity and isotropy, as well as spatially flat Cauchy slices leads to the following modified Friedmann equation
\begin{equation}
3H_{ f(R)}^{2}=\frac{f_{R}\left[2 \kappa^{2} \rho+{R} f_{R}-f\right]}{2\left(f_{R}+\frac{f_{R R}}{2} \frac{\dot{R}}{H}\right)^{2}}.\label{fRFriedmann}
\end{equation}
where $\kappa^2=8\pi G$ and we have the following relations valid in any metric-affine $f(R)$ theory
\begin{align}\label{fRrelations}
\rho=\frac{R f_R-2f(R)}{2\kappa^2}\qquad\text{and}\qquad\frac{\dot{R}}{H}=-12\kappa^2 \rho/(R f_{RR}-f_{R}),
\end{align}
By imposing equality between the Hubble parameter of $f(R)$ and the corresponding Loop cosmology, we can derive the conditions for $f(R)$ to describe a background evolution that is equivalent to such Loop cosmology. Using then the above relation between the energy density, $f(R)$ and its derivative  $f_R$ in such equality, one is led to a 2nd order highly non-linear ODE for $f(R)$ which for the three Loop cosmology models that we will be concerned with can be encoded into the following form
\begin{equation}\label{generalODE}
f_{RR}=f_R\left(\frac{B \Delta-f_{R}A}{B\Delta R+2A(R f_{R}-3f)}\right)
\end{equation}
where $A$, $B$ and $\Delta$ are functions of $R$, $f(R)$, $f_R$ that are different for each Loop Cosmology model. Physical equivalence between the Loop and $f(R)$ bounces requires equivalence of the bounce densities in both frameworks, which allow us to obtain boundary conditions for the ODE. Given the uniqueness theorems of ODEs, this leads to a particular $f(R)$ solution to each of the models. For the three models, the only consistent boundary condition for $f_R$ at the bounce is $f^\textrm{b}_R=0$, where the superindex b stands for bounce. The ODEs have to be solved numerically due to their complexity, but the boundary condition $f^\textrm{b}_R=0$ cannot be handled by numerical methods for equations of the form \eqref{generalODE}. Assuming that uniqueness theorems hold throughout the whole range of curvatures $R\in(-\rb,0)$, namely that the quotient is regular throughout this interval\footnote{Actually, we have checked that this is true numerically for each of the solutions.}, we can chose to place boundary conditions anywhere. Except for the pre-bounce phase of mLQC-I,  we generally go for boundary conditions at low curvatures because we know that the solution should reduce to GR in the low curvature limit, and it proves to be easier to find the solution giving a correct bounce density\footnote{We also tried near-bounce conditions for LQC, finding the same solution as boundary conditions at low $R$.} with the initial conditions placed there. The values of the energy density and $f(R)$ at the bounce are extremely sensitive to the initial conditions for the derivative at low curvatures, and there exists a critical value for $f_{R}^\textrm{boundary}$ which, if surpassed, leads to a solution that is not regular through the whole curvature range, spoiling the certainty of uniqueness of the solution. Although the correct solutions for LQC and mLQC-II clearly satisfy the conditions of the uniqueness theorems\footnote{Meaning that the boundary conditions for $f_R$ that lead to the correct bounce density are below the critical value and the solutions and ODE are suitably regular from low curvatures to the bounce.}, this is not the case for mLQC-I, where all seems to indicate that the would-be solution with the correct bounce density has a divergence of $f_{RR}$ exactly at the bounce as we will see below. As a remark, note that if uniqueness theorems are satisfied, the existence of a solution to the ODE that satisfies the required conditions at the bounce but also satisfies $\lim_{R\to0}f_R=1$ is far from being guaranteed, but indeed a surprising feature that indicates that either the bounce boundary conditions or the $R=0$ conditions are attractors of the corresponding ODEs. To be more explicit, a regular ODE in a given range of values for the relevant variable, its solution is unique as guaranteed by the corresponding uniqueness theorems. Thus, once boundary conditions for $f(R)$ and $f_R$ are specified at some point within such range, the solution in the full range is unique, and it is likely not to pass through another point given beforehand unless this is an attractor in solution space. For instance, if conditions are set at the bounce, it is likely that no solution with the correct behaviour at low curvatures exists. Given that the bounce is a regular point for both LQC and mLQC-II, $f_R|_{R=0}=1$  is probably an attractor for the three ODEs.


\subsection{ODE and numerical solution for LQC}

The modified Friedmann equation that describes LQC evolution (for a massless scalar) is given by 
\begin{equation}
3H_\textrm{LQC}^2=\kappa^2\rho\lr{1-\frac{\rho}{\rhob}},
\label{LQCFriedmann}
\end{equation}
where $\rhob\equiv\sqrt{3}/(16\pi^2\gamma^3G^2\hbar)$ and $\gamma$ is the Barbero-Immirzi parameter. By equating this expression for the Hubble rate with the one given in \eqref{fRFriedmann} and using \eqref{fRrelations} to write $\dot R/H$ and $\rho$ in terms of $R$, $f(R)$ and $f_R$, we arrive at an ODE of the form \eqref{generalODE} with the particular form of the functions
\begin{equation}\label{LQCODEfunctions}
\begin{split}
&A_\textrm{LQC}=\sqrt{2\left({R} f_{R}-2 f\right)\left(2{R}_{\textrm{c}}-\left({R} f_{R}-2 f\right)\right)},\\
&B_\textrm{LQC}=2\sqrt{{R}_{\textrm{c}} f_{R}\left(2 {R} f_{R}-3 f\right)},\\
&\Delta_\textrm{LQC}=1.
\end{split}
\end{equation}
The conditions that the bounce density and the bounce accelerations of the scale factor coincide at the bounce in the LQC and $f(R)$ side lead to a set of conditions with a unique physically relevant solution given by
\begin{align}\label{LQCboundcond}
&f(R_\textrm{b})= -\rc\qquad\text{and}\qquad f_R(R_\textrm{b})= 0,
\end{align}
where the bounce curvature is
\beq
R^\textrm{LQC}_\textrm{b}=-12R_{\textrm{c}}
\eeq
and $\rc\equiv \kappa ^2 \rho_{\textrm{c}}$ and $\rho_{\textrm{c}}$ is the LQC bounce density. As explained above, the ODE has to be solved numerically, and the theoretical boundary conditions \eqref{LQCboundcond} are not well suited for numerical solving due to the form of the ODE. Using suitable boundary conditions, we find a solution for LQC which satisfies the uniqueness criteria and gives the correct bounce density with a precision of up to seven digits. This solution is the same as the one found in \cite{Olmo:2008nf}, and we have also been able to reproduce it by fixing boundary conditions near the bounce. We will later see how this solution is acurately reproduced by an analytical $f(R)$ Lagrangian that fits within a 3-parameter family of Lagrangians and coincides with the one found in \cite{Olmo:2008nf}.


\subsection{ODE and numerical solution for mLQC-II}


 As standard LQC, mLQC-II describes a symmetric bounce through a modified Friedmann equation given by \cite{Li:2018fco,Li:2018opr}
\begin{equation}
3H^2_{\textrm{II}}=\kappa^2 \rho\left(1+\gamma^{2} \frac{\rho}{\rho_{c}}\right)\left(1-\frac{\left(\gamma^{2}+1\right) \rho / \rho_{c}}{\left(1+\sqrt{\gamma^{2} \rho / \rho_{c}+1}\right)^{2}}\right)
\label{mLQC-IIFriedmann}
\end{equation}
Proceeding as for the LQC case above, by equating the above expression for the Hubble parameter and the one in $f(R)$ \eqref{fRFriedmann}, using \eqref{fRrelations} we also obtain an ODE of the form \eqref{generalODE} with the following functions
\begin{equation}
\begin{split}
&A_{\textrm{II}}=\sqrt{2\left({R} f_{R}-2 f\right)\left(2{R}_{\textrm{c}}+\gamma^2\left({R} f_{R}-2 f\right)\right)},\\
&B_{\textrm{II}}=B_\textrm{LQC}=2\sqrt{{R}_{\textrm{c}} f_{R}\left(2 {R} f_{R}-3 f\right)},\\
&\Delta_{\textrm{II}}=\sqrt{\frac{\gamma^2\left(1+\sqrt{\gamma^2\frac{R f_R-2f}{2R_{\textrm{c}}}+1}\right)}{2\gamma^2+1-\sqrt{\gamma^2\frac{R f_R-2f}{2R_{\textrm{c}}}+1}}},
\end{split}
\end{equation}
where note that, in a purely formal way, by substituting $\gamma^2$ by $-1$, the above functions become the ones obtained for LQC in \eqref{LQCODEfunctions}. The requirements that the solutions have the same energy density and acceleration of the scale factor at the bounce completely specify the boundary conditions, which read
\begin{align}
&f(R^{\textrm{II}}_{b})=-4 R_{\textrm{c}}(1+\gamma^2)\quad\text{and}\quad f_{R}(R^{\textrm{II}}_\textrm{b})=0,
\end{align}
where the bounce curvature is 
\beq
R^{\textrm{II}}_\textrm{b}=-48 (1+\gamma^2)(1+2\gamma^2)R_{\textrm{c}},
\eeq
 and the bounce density in mLQC-II is given by $\rho^{\textrm{II}}_\textrm{b}=4(1+\gamma^2)\rho_{\textrm{c}}$. With these conditions, we can obtain a numerical solution that seems to satisfy all the required criteria for the uniqueness theorems to apply in the relevant curvature range, see Fig. \ref{fig:1stfitsLQC}. The sensitivity of the bounce density to the initial conditions as well as the stability of the solutions have similar behaviour as the LQC case. 



\subsection{ODE and numerical solution for mLQC-I}

Unlike LQC and mLQC-II, mLQC-I describes an asymmetric bounce where the contracting and expanding branches are described respectively by the two modified Friedman equations below. The bounce density in mLQC-I is given by $\rho^{\textrm{I}}_\textrm{b}=\rho_{\textrm{c}}/(4(1+\gamma^2))$ and this implies the following value for the affine curvature at the bounce and boundary conditions
\begin{align}\label{BounceRI}
&R^{\textrm{I}}_\textrm{b}=- \frac{3(1+2\gamma^2)}{(1+\gamma^{2})^2}R_{\textrm{c}},\\
&f(R^{\textrm{I}}_{b})= \frac{R_{\textrm{c}}}{4(1+\gamma^2)}\quad\text{and}\quad f_{R}(R^{\textrm{I}}_\textrm{b})=0.
\end{align}
We can attempt the finding of a numerical solution for each of the branches.\\

\subsubsection{Post-bounce phase (-)}

The cosmological evolution of the post-bounce phase of mLQC-I is described by the modified Friedmann equation \cite{Li:2018fco,Li:2018opr}
\begin{equation}
3H^2_{\textrm{I}-}=\kappa^2\left(1-\frac{\rho}{\rhob^{\textrm{I}}}\right)\left[1+\frac{\gamma^2}{1+\gamma^2}\left(\frac{\sqrt{\rho/\rhob^{\textrm{I}}}}{1+\sqrt{1-\rho/\rhob^{\textrm{I}}}}\right)\right],
\label{mLQC-IFriedmann}
\end{equation}
Again, by equating the above expression for the Hubble rate to the one in $f(R)$ theories \eqref{fRFriedmann} we arrive to an ODE of the general form \eqref{generalODE}, with the particular values of the functions
\begin{equation}
\begin{split}
&A^-_{I}=\sqrt{2(R f_{R}-2f)\left(\frac{R_{\textrm{c}}}{2(1+\gamma^2)}-R f_{R}+2f\right)}\\
&B_{I}=\sqrt{\frac{{R}_{\textrm{c}}}{1+\gamma^2} f_{R}\left(2 {R} f_{R}-3 f\right)}\\
&\Delta^-_{I}=\sqrt{\frac{R_{\textrm{c}}-(1+\gamma^2)(R f_R-2f)+\sqrt{R_{\textrm{c}}^2-2(1+\gamma^2)R_{\textrm{c}}(R f_{R}-2f)}}{(1+\gamma^2)\left(R_{\textrm{c}}+2f-R f_R+\sqrt{R_{\textrm{c}}^2-2(1+\gamma^2)R_{\textrm{c}}(R f_{R}-2f)}\right)}}\\
\end{split}
\end{equation}
We have obtained a numerical solution that matches the boundary conditions \eqref{BounceRI}. This solution can be seen in Fig. \ref{fig:1stfitsLQC}. This ODE shows the same issues with sensitivity to the initial value and stability as the other cases. However, there is a qualitative difference with respect to LQC and mLQC-II: in this case the second derivative of $f(R)$ diverges at the bounce with an asymptotic dependence of the form $(R-R_\textrm{b})^{-1/2}$.\\ 

We also find the following: For boundary conditions leading to bounce densities which are much lower than the correct value, the convergence of the numerical solver extends to arbitrarily large curvatures. However, although we can obtain values of the bounce density for the numerical solution which are very close to the correct bounce densities, for bound densities close enough to the correct value, the convergence range ODE develops an upper limit at some value of the affine curvature greater than the bounce curvature. The curvature at which this happens quickly approaches the bounce curvature when the boundary conditions approach those that give the correct bounce density. Numeric experiments appear to suggest that this upper limit is the bounce curvature itself for the solution that would give exactly the correct bounce density, thus spoiling uniqueness. Hence, it appears that the boundary conditions leading to a correct bounce density, namely \eqref{BounceRI}, are a singular point in the solution space of the ODE describing mLQC-I and $f(R)$ equivalence.

\subsubsection{Pre-bounce phase (+)}

The cosmological evolution of the pre-bounce phase of mLQC-I is described by the modified Friedmann equation\cite{Li:2018fco,Li:2018opr}
\begin{equation}
3H^2_{\textrm{I}+}=\kappa^2 \alpha \rho_{\Lambda}\left(1-\frac{\rho}{\rhob^\mathrm{I}}\right)\left[1+\frac{1-2\gamma^2+\sqrt{1-\rho/\rhob^\mathrm{I}}}{4\gamma^2(1+\sqrt {1-\rho/\rhob^\mathrm{I}})}\frac{\rho}{\rhob^\mathrm{I}}\right],
\label{mLQC-IpreFriedmann}
\end{equation}
where $\alpha=(1-5\gamma^2)/(1+\gamma^2)$, $\rho_{\Lambda}=3/(\kappa^2\alpha\lambda^2(1+\gamma^2)^2)$ and $\lambda^2=\sqrt{3}\kappa^2 \gamma/2$.  Again, by equating the above expression for the Hubble rate to the one in $f(R)$ theories \eqref{fRFriedmann} we arrive to an ODE of the general form \eqref{generalODE}, with the particular values of the functions 
\begin{equation}
\begin{split}
&A^+_{I}=\sqrt{\frac{4 \sqrt{3} \left(\frac{\rc}{2 \left(\gamma ^2+1\right)}-R f'(R)+2 f(R)\right)}{\left(\gamma ^2+1\right) \gamma   \kappa ^2 R_{\textrm{c}}}},\\
&B^+_{I}=\sqrt{\frac{{R}_{\textrm{c}}}{1+\gamma^2} f_{R}\left(2 {R} f_{R}-3 f\right)},\\
&\Delta^+_{I}=\sqrt{\frac{\gamma^2\left(\sqrt{\frac{R_{\textrm{c}}}{2(1+\gamma^2)}}+\sqrt{\frac{R_{\textrm{c}}}{2(1+\gamma^2)}-R f_{R}+2f}
\right)}{2\gamma^2+1-\sqrt{\frac{R_{\textrm{c}}}{2(1+\gamma^2)}-R f_{R}+2f}
}}.\end{split}
\end{equation}

Though we know the boundary conditions at the bounce, these are not well suited for numerical solving. This was also the case for the post-bounce branch and the other two models, but in those cases we knew that the boundary conditions at low curvatures must be compatible with the metric-affine Einstein-Hilbert action to a high degree of approximation. Here, however, the prebounce phase does not need to be arbitrarily close to GR at low curvatures (we actually do not have any physical information about the prebounce phase). Thus, it is not yet clear how to attempt a numerical solution. Steps to solve this issue are currently being undertaken. 

\section{An $f(R)$ family for Looping them all}

In the original paper by Olmo and Singh \cite{Olmo:2008nf}, an analytic approximation to the standard LQC numerical solution of the ODE defined by \eqref{LQCODEfunctions} with boundary conditions \eqref{LQCboundcond} was given as
\begin{equation}\label{BestFitLQC}
f({R})=\frac{{R}}{12}\left(1-\frac{1}{2} \ln \left[\left(\frac{{R}}{12{R}_{c}}\right)^{2}\right]\right)+\frac{{R}\left({R}+12 {R}_{c}\right)^{2}}{6500 {R}_{c}^{2}}
\end{equation}
Following their work, we would like now to find an analytic covariant function that describes the different Loop cosmologies. We will do so by generalising the above function. Let us try the generalised ansatz consisting on the following 3-parameter family of metric-affine $f(R)$ Lagrangians
\begin{equation}\label{GenericModel}
f(R)=\xi R\left[1+\frac{(\alpha R_{\textrm{c}}+R)^2}{\beta \alpha^2 R_{\textrm{c}}^2}-\frac{1}{2}\ln\left(\frac{R^2}{\alpha^2 R_{\textrm{c}}^2}\right)\right].
\end{equation}
Here, the parameter $\alpha$ determines the bounce affine curvature in units of $R_{\textrm{c}}$, $\xi$ determines the value of the Lagrangian at the bounce for a given $\alpha$, and $\beta$ is a free parameter with the condition $\beta\geq2$ so that the derivative of the Lagrangian does not vanish within the interval $R\in(-R_\textrm{b},0)$. By requiring that this Lagrangian is compatible with the bounce conditions of LQC, mLQC-I and mLQC-II already fixes $\alpha$ and $\xi$ in the three cases to be
\begin{align}\label{CoeffVal}
\begin{split}
&\alpha_\textrm{LQC}=12, \hspace{1cm} \alpha^-_{\textrm{I}}=\frac{3 (1+2\gamma^2)}{(1+\gamma^2)^2}, \hspace{1cm} \alpha_{\textrm{II}}=48(1+2\gamma^2)(1+\gamma^2),\\
&\xi_\textrm{LQC}=\frac{1}{\alpha_\textrm{LQC}},\hspace{1cm}\xi^-_{\textrm{I}}=\frac{1}{4(1+\gamma^2)\alpha_{\textrm{I}}}, \hspace{1cm} \xi_{\textrm{II}}=\frac{4(1+\gamma^2)}{\alpha_{\textrm{II}}}.
\end{split}
\end{align}
\begin{figure}[h]
\centering
\includegraphics[width=0.32\textwidth]{Figures/LQC/BestFitLQC}
\includegraphics[width=0.32\textwidth]{Figures/LQC/BestFitLQCder}
\includegraphics[width=0.32\textwidth]{Figures/LQC/BestFitLQC2der}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitI}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitIder}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitI2der}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitII}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitIIder}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitII2der}
\caption{Plot of the analytical approximation \eqref{BestFitLQC} with $\beta$ given in \eqref{betafits} and the numerical solution to the corresponding ODE \eqref{generalODE}. We plot $f(R)$, $f_R$, $f_{RR}$. The first row is standard LQC, the second is the postbounce branch of mLQC-I and the third is mLQC-II.}
\label{fig:1stfitsLQC}
\end{figure}
By using these values, and minimising the area between the numerical solution and the analytic approximation, we can find a best fit for the parameter $\beta$ for each of the models. The best fit values are 
\begin{align}\label{betafits}
&\beta_\textrm{LQC}=3.84 \hspace{1cm} \beta_{\textrm{I}}^{-}=4.77 \hspace{1cm} \beta_{\textrm{II}}=3.10.
\end{align}
In figure \ref{fig:1stfitsLQC}, the analytic approximation \eqref{BestFitLQC} and the numerical solution to \eqref{generalODE} with the corresponding functions and boundary conditions, as well as their derivatives are plotted for the corresponding values of $\alpha$ and $\xi$, given in \eqref{CoeffVal}, and the above best fit values of $\beta$. In figure \ref{fig:1stfitsLQCdens} the same is done with the energy density normalised at the bounce. We can see how the analytic approximations fit the numerical solution up to deviations of at most around 1\% from low curvatures almost up to the bounce in the energy density profile of the three models. Though the bounce is perfectly captured in both LQC and mLQC-II, in mLQC-I the second derivative $f_{RR}$ blows up when approaching the bounce. By performing numerical experiments, we can see how this divergence goes asymptotically like $(R-R_\textrm{b})^{-1/2}$. This behaviour can be seen also in $\rho$ which does not approach the bounce with the correct asymptotic behavior. This issue can be solved by adding a $(R-R_\textrm{b})^{3/2}$ term to the generic form for $f(R)$ in \eqref{GenericModel}.  As well, we can design {\it ad hoc} polynomial corrections to mLQC-I and -II separately that reduce the deviations to the 0.1\% level.




\begin{figure}[h]
\centering
\includegraphics[width=0.32\textwidth]{Figures/LQC/BestFitLQCdens}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitIdens}
\includegraphics[width=0.32\textwidth]{Figures/LQC/FirstAnalitycFitIIdens}
\label{fig:1stfitsLQCdens}
\caption{Plot of the energy density normalised at the bounce for the analytical approximation \eqref{BestFitLQC} of each model with $\beta$ given in \eqref{betafits} and the numerical solution to the corresponding ODE \eqref{generalODE}. The first row is standard LQC, the second is the postbounce branch of mLQC-I and the third is mLQC-II.}
\end{figure}



\subsubsection{Corrections to the generic Lagrangian}


To make the generalised model \eqref{GenericModel} account for the $(R-R_\textrm{b})^{-1/2}$ divergence of $f_{RR}$ at the bounce, as well as the 1\% deviations in the energy density profile, we modify it by
 \begin{equation}\label{eq:BestfitIpost}
\begin{split}
f_-^{\textrm{I}}(R)=&\xi R\left[1+\frac{(\alpha R_{\textrm{c}}+R)^2}{\beta \alpha^2 R_{\textrm{c}}^2}-\frac{1}{2}\log\left(\frac{R^2}{\alpha^2 R_{\textrm{c}}^2}\right)\right]+\frac{8 \epsilon}{3 \beta \alpha}\sqrt{\frac{(R+\alpha \rc)^3}{\alpha \rc}}-\\
-&\tilde\epsilon\left[\frac{(R-\alpha\rc)^2}{10}\left(1-\frac{R-\alpha\rc}{10}\right)-\frac{1}{2}R(R-\alpha\rc)\left(R-\frac{\alpha\rc}{3}\right)\right],
\end{split}
\end{equation}
and for mLQC-II we add polynomial corrections without the divergent term of the form
\begin{equation}\label{BestAnalyticII}
\begin{split}
f^{\textrm{II}}(R)=&\xi R\left[1+\frac{(\alpha R_{\textrm{c}}+R)^2}{\beta \alpha^2 R_{\textrm{c}}^2}-\frac{1}{2}\ln\left(\frac{R^2}{\alpha^2 R_{\textrm{c}}^2}\right)\right]+\tilde\epsilon\frac{R}{10^5} \Bigg[\frac{3}{50} R^4+ \left(\frac{29}{200} \alpha \rc+\frac{5}{6}\right) R^3\\
&+\alpha \rc \left(\frac{71}{600}\alpha\rc+\frac{16}{3}\right)R^2+\alpha^2\rc^2 \left(\frac{\alpha\rc}{25}+\frac{13}{4}\right)R+ \alpha^3 \rc^3 \left(\frac{\alpha\rc}{200}+\frac{1}{2}\right) \Bigg]
\end{split}
\end{equation}
where $(\alpha,\xi)$ are also given by \eqref{CoeffVal} and have the same meaning in both cases, the parameter controlling the bounce divergence of $f_{RR}$ in mLQC-I is $\epsilon=10^{-2}$, and the coefficients of the polynomial proportional to $\tilde\epsilon$ are at most of order 1 with $\tilde\epsilon=10^{-2}$. $\beta$ is again a free parameter that allows to fit the numerical solution. We obtain almost the same best-fit value for $\beta$ as without the correction, namely $\beta_{\textrm{I}}=4.76$ and $\beta_{\textrm{II}}=2.70$. As can be seen in figure \ref{fig:BestFitmod}, the fit of the analytical normalised energy density to the numerical solution improves respect to the general form \eqref{GenericModel} in both cases, and the divergence of $f_{RR}$ in mLQC-I is captured accurately (see figure \ref{fig:BestFitmod2der}).
\begin{figure}
\includegraphics[width=0.48\textwidth]{Figures/BestFitIIdens}
\includegraphics[width=0.48\textwidth]{Figures/BestFitIdens}
\caption{Plots of the energy density normalised at the bounce for mLQC-I and -II after the improved version of the respective analytic approximations \eqref{eq:BestfitIpost} and \eqref{BestAnalyticII}. We also plot the corresponding numerical solution. }
\label{fig:BestFitmod}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.48\textwidth]{Figures/BestFitI2der}
\label{fig:BestFitmod2der}
\caption{Plot of $f_{RR}$ for the improved analytical approximation to mLQC-I from \eqref{eq:BestfitIpost} with $\beta_{\textrm{I}}^-=4.76$ and the corresponding numerical solution. The divergent behaviour is captured perfectly.} 
\end{figure}
To close up, we have seen how the background evolution of isotropic and homogeneous models of Loop Cosmologies can be mimicked precisely by metric-affine $f(R)$ theories. Even more, these theories are not completely different for each of the models, but they rather obey the general nonperturbative behaviour of a family of metric-affine $f(R)$ theories given by \eqref{GenericModel}. This result is rather remarkable as, even though the three Loop Cosmology models stem from a common framework and differ due to quantisation ambiguities in isotropic and homogeneous spacetimes, the $f(R)$ theories could all have a different nonperturbative behavior. Nevertheless, we have shown how this is not the case, and the $f(R)$ models describing the three Loop Cosmologies originate from the same functional dependence on the affine curvature, each model differing only in the value of the corresponding parameters. This reminds to the situation where one derives an effective field theory for general Loop Cosmologies, which would only differ on the value of the different Wilson coefficients, thus suggesting that $f(R)$ theories could be capturing some nonperturbative features of LQG. This suggests the study of this family of theories in other scenarios such as anisotropic cosmologies or spherically symmetric spacetimes to see if it can also describe their Loop quantised versions. As well, confronting this family with Loop Cosmologies at the level of perturbations, or trying to find an improved one which does a better job if this one fails, is also an important direction to be explored in the future.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

			%NEWCHAPTER%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{Spontaneous Lorentz symmetry breaking in the metric-affine framework}\label{sec:SLSB}


The consistent inclusion of Lorentz symmetry breaking in a curved space is currently an open problem, though it is motivated by several approaches to find the UV completion of GR \cite{Colladay:1996iz,Gambini:1998it,Amelino-Camelia:2001dbf,Alfaro:2004aa,Bojowald:2004bb,Calcagni:2016zqv}. The usual way of including explicit Lorentz symmetry breaking by introducing a constant privileged direction cannot be generalised in a straightforward manner in presence of a nontrivial gravitational background while respecting diffeomorphism covariance. This is due to the fact that the partial derivative operator is tied to a given coordinate system, and it is not covariant when acting on generic tensor fields (see chapter {\ref{sec:DifferentialGeometry}}). Covariant differential operators that could be used to implement the constant condition could be $\dif$ or $\nabla$. If the privileged direction is defined by a vector $b$, imposing the vanishing of $\dif b$ would lead to $b=\dif \phi$ for a given scalar $\phi$, which is not a Lorentz violating constraint. By imposing $\nabla b=0$ we end up with a constraint equation for the connection, or the metric if we do it in the metric formalism, which is not generally acceptable from the physical viewpoint.

Another possibility is thus to resort to a spontaneous breaking of Lorentz symmetry via a vacuum expectation value of some field which belongs to some representation of the Lorentz group which is not the trivial one. The easiest way to go is by considering a vector field with a potential that leads to the existence of stable nontrivial vacua so that the vacuum expectation value (VEV) of the field breaks Lorentz symmetry spontaneously. This was done in presence of gravity by Kostelecky in what is known as the Bumblebee model \cite{Kostelecky:2003fs}, where a coupling of the vector field to the Ricci tensor is considered. Several aspects of this model have been studied over the years, all within the Riemannian framework \cite{Bertolami:2005bh,Seifert:2009gi,Maluf:2014dpa,Santos:2014nxm,Casana:2017jkc,Oliveira:2018oha,Ovgun:2018ran,Ovgun:2018xys,Ding:2019mal,Kanzi:2019gtu,Chen:2020qyp,Li:2020wvn,Maluf:2020kgf,Maluf:2021lwh,Oliveira:2021abg,Assuncao:2019azw}. As well, experimental tests of Lorentz violating extensions of the Standard Model and GR have led to stringent constraints on Lorentz breaking parameters \cite{Bailey:2006fd,Kostelecky:2008ts,Kostelecky:2015dpa,Kostelecky:2016kfm}. As a first step to study spontaneous symmetry breaking of Lorentz symmetry within the metric-affine framework, in this chapter we will consider a metric-affine formulation of the Bumblebee model \cite{Delhom:2019wcm,Delhom:2020gfv}. 

As we will see, this fits perfectly into the framework of RBG theories already developed in chapter \ref{sec:RBGTheory}. Indeed, due to the fact that the Ricci tensor appears only linearly in the Lagrangian, this will be a particularly easy example of Ricci-Based theory with projective symmetry and nonminimal couplings between matter and geometry. As we will see, the resulting theory admits an exact formal solution for the independent connection which leads to the emergence of a nonmetricity tensor generated by the nonminimal Bumblebee coupling to the geometry, which in the Einstein frame will couple to the rest of the matter fields present in the theory due to $Q$-induced interactions. We will first analyse briefly the structure of the theory, building the corresponding Einstein frame.  In the weak gravitational field limit, and perturbatively in the nonminimal coupling constant, we will study the stability of the Bumblebee vacua. Then, assuming a generic vacuum for the Bumblebee field, which should be particularised to the stable one for practical applications, we study the resulting field equations for scalar and Dirac fields, focusing on the Lorentz violating parameters and their modified dispersion relations. 



\section{The Metric-Affine Bumblebee model}

We will consider a metric-affine Bumblebee model where the only nonminimal coupling to the geometry occurs through the Bumblebee field. This model is described by a Lagrangian of the form 
\begin{eqnarray} 
\nonumber\mathcal{L}=R+\frac{2\xi}{{\mq^2}} B^{\mu} B^{\nu} R_{\mu\nu}+ \frac{2}{{\mpl^2}}\lrsq{-\frac{1}{4}B^{\mu\nu}B_{\mu\nu}-V(B^{\mu}B_{\mu}\pm b^2) +\mathcal{L}^{\textrm{MC}}_{\textrm{m}}\big(g_{\mu\nu},\Psi_i)}.
\label{Bumblebee}
\end{eqnarray}
Here $B_{\mu\nu}=(\mbox{d}B)_{\mu\nu}$, and  we have written the Bumblebee piece of the action separated from the minimally coupled piece of the matter sector $\mathcal{L}^{\textrm{MC}}_{\textrm{m}}$, and we have neglected the fermion couplings to torsion so that $\mathcal{L}^{\textrm{MC}}_{\textrm{m}}$ does not depend on the connection and the effects of the Bumblebee nonminimal coupling appear more transparent\footnote{Indeed, adding the fermionic minimal coupling to torsion only adds a linear coupling to the connection in the spinorial sector of $\mathcal{L}^{\textrm{MC}}_{\textrm{m}}$. This would lead to a Planck-scale suppresed four-fermion contact interaction which we will neglect for the same reasons as in chapter \ref{sec:ObservableTraces}.\label{foot1Bumb}}.  The potential of the Bumblebee field $B_\mu$ guarantees that there are nontrivial Bumblebee vacua which spontaneously break Lorentz symmetry by introducing a privileged direction. 

The above action is within the class described by \eqref{eq:GeneralRBGAction} with a nonminimal coupling of the matter sector to the geometry through the Bumblebee field controlled by the dimensionless coefficient $\xi$. Following the reasoning in chapter \ref{sec:RBGTheory}, we find that the connection field equations of \eqref{Bumblebee} are an algebraic constraint, so that the connection is an auxiliary field that can be algebraically solved as the canonical connection of the Einstein frame metric
\begin{align}
 \sqrt{-q}q^{\mu\nu}=g^{\mu\nu}+\frac{2\xi}{{\mq^2}} B^\mu B^\nu.\label{eq:AuxMetricBumb}
\end{align}
This relation allows us to fin  $\beta_g^2=g^{\mu\nu}B_{\mu}B_{\nu}$, in terms of $\beta_q^2=q^{\mu\nu}B_{\mu}B_{\nu}$ as
\beq\label{eq:SolutionSquaredBumb}
\beta^2_q=\beta^2_g\sqrt{1+\frac{2\xi}{{\mq^2}}\beta_g}
\eeq
 which can be solved algebraically to find $\beta_g^2(\beta_q^2)$, leading to
 the expression of $g_{\mu\nu}$ in terms of $q_{\mu\nu}$ and the Bumblebee field as
\begin{equation}\label{eq:gmn_0}
\begin{split}
g_{\mu\nu}=\frac{1}{\sqrt{1+\frac{2\xi}{{\mq^2}} \bar\beta^2}}q_{\mu\nu}+\frac{2\xi}{{\mq^2}}\frac{1}{1+\frac{2\xi}{{\mq^2}} \bar\beta^2}B_{\mu}B_{\nu} \ ,\end{split}
\end{equation}
where we have called $\bar\beta^2$ to the solution $\beta_g^2(\beta_q^2)$ of \eqref{eq:SolutionSquaredBumb} and we can find $g^{\mu\nu}$ by inverting the above equation as a matrix equation. Proceeding as in section \ref{sec:EinsteinFrame}, we arrive to the Einstein frame form of the Bumblebee action \eqref{Bumblebee}, which reads
\begin{eqnarray} 
\nonumber\mathcal{L_{\textrm{EF}}}=R+\frac{2}{{\mpl^2}}\bar{\mathcal{L}}^\xi_{\textrm{m}}\big(q_{\mu\nu},B_\mu,\Psi_i\big)
\label{EinsteinBumblebee}
\end{eqnarray}
where any barred tensor indicates that its indices are raised and lowered with $q^{\mu\nu}$, so that the $g_{\mu\nu}$ metrics have been substituted by $q_{\mu\nu}$ through \eqref{eq:gmn_0} and its inverse. We have now included the bumblebee terms within $\bar{\mathcal{L}}^\xi_{\textrm{m}}$, which is denoted by the superscript $\xi$. In the above form, it is apparent that, due to the fact that it belongs to the (nonminimally coupled) RBG subclass of metric-affine theories, the Bumblebee model can be interpreted as GR coupled to a modified matter sector in which all the matter fields couple to the Bumblebee through $Q$-induced interactions with coupling strength $\xi/{\mq^2}$, including new self-interactions that modify the Bumblebee potential. 

According to the above form of the Bumblebee action, the metric $q_{\mu\nu}$ satisfies the Einstein equations coupled to a highly non-linear matter sector. Therefore, $q_{\mu\nu}$ will depart from the Minkowski metric only in regions where the Newtonian and post-Newtonian effects are expected to be relevant, \ie regions with a strong gravitational field. As a result, as it follows from (\ref{eq:gmn_0}), the metric $g_{\mu\nu}$ will not only describe the two propagating degrees of freedom corresponding to a massless spin-2 field described by $q_{\mu\nu}$, but it will also encode information on the local value of the Bumblebee field via a conformal factor and a disformal term proportional to $B_{\mu}B_{\nu}$ both of which source nonmetricity as can be seen by noting that the connection field equations are solved by the constraint  $\nabla_\alpha q^{\mu\nu}=0$. Thus, the nonmetricity tensor is nontrivial, controled by $\xi/{\mq^2}$, and entirely due to the covariant derivatives of the Bumblebee field. Since this field is expected to have a nontrivial VEV that spontaneously breaks Lorentz invariance, this is an example of a gravitationally generated nonmetricity tensor that can develop a VEV. In contrast, in RBGs with minimally coupled matter, the nonmetricity is associated to derivatives of the stress-energy tensor of the matter fields, which vanish in vacuum. Within the assumption that there is a constant nonmetricity background around the Earth, experimental constraints to all the possible effective couplings between fermions and photons and nonmetricity were derived from Lorentz violation searches within Earth laboratories in \cite{Foster:2016uui}. Since minimally coupled matter fields do not couple explicitly to nonmetricity, these constraints do not apply to our model. However, this model provides an explicit example of a gravitational model with a nontrivial nonmetricity VEV that the author knows of. Furthermore, note that constraints on Lorentz-violating couplings such as those in the Standard Model Extension \cite{Bailey:2006fd} could translate into constraints on the Bumblebee nonminimal coupling $\xi$. Below, we will facilitate the translation of these bounds by deriving the effective Klein-Gordon and Dirac equations in presence of a nontrivial Bumblebee VEV. 
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\section{Weak gravitational field limit}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
We can now explore the weak gravitational field limit of the model, so that the effects of the Bumblebee couplings to matter appear transparently. This limit would be applicable in \eg non-gravitational experiments on Earth's surface, where all Newtonian and post-Newtonian corrections to the Minkowski metric can be safely neglected. Given that $q_{\mu\nu}$ satisfies Einstein's equations, this amounts to the approximation $q_{\mu\nu}\approx\eta_{\mu\nu}$, in the same spirit as in chapter \ref{sec:ObservableTraces}. Considering also $\xi$ as a small coupling, we can write the following perturbative relations between both metrics
\begin{equation}
\begin{split}
g^{\mu\nu}=\eta^{\mu\nu}-\frac{2\xi}{{\mq^2}}\lr{B^{\mu}B^{\nu}-\frac{1}{2}B^{\alpha}B_{\alpha}\eta^{\mu\nu}}+\mathcal{O}\lr{\frac{\xi^2}{{\mq^4}}}
\label{efmet}
\end{split}
\end{equation}
where we now raise and lower indices with the Minkowski metric consistently with our approximations. This expression will allow us to write the Einstein frame effective Lagrangians and field equations for the Bumblebee field, as well as for scalar and Dirac matter fields. 
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effective dynamics for matter fields}
%%%%%%%%%%%%%%%%%%%%%%
Proceeding in similar lines as in section \ref{sec:NMLag}, we can find the effective Lagrangians describing scalar and Dirac fields perturbatively in $\xi/{\mq^2}$, which are given by
\begin{align}
&\resizebox{.9\hsize}{!}{$\mathcal{L}_{(0)}=-\frac{1}{2}\Phi(\Box_\eta+m^2)\Phi+\frac{\xi}{{\mq^2}}\Phi\Big[B^{\mu}B^{\nu}\partial_{\mu}\partial_{\nu}+ \big(B^\mu (\partial_\nu B^\nu)+B^\nu (\partial_\nu B^\mu)\big)\partial_\mu+\frac{m^2}{2} B^2\Big]\Phi+\mathcal{O}\lr{\frac{\xi^2}{{\mq^4}}}$},\label{31}\\
&\resizebox{.9\hsize}{!}{$\mathcal{L}_{(1/2)}=\bar\Psi(i \gamma^\mu \partial_\mu-m) \Psi-\frac{\xi}{{\mq^2}} \bar\Psi\Bigg[\frac{i}{2} B^{2} \gamma^\mu \partial_{\mu}+i B^\mu B^{\nu} \gamma_{\mu} \partial_{\nu}+\frac{i}{2}\Big(B_{\alpha}\left(\partial_{\mu} B^{\alpha}\right)+B^{\nu}\left(\partial_{\nu} B_{\mu}\right)+(\partial_\alpha B^\alpha) B_{\mu}\Big) \gamma^{\mu}-m B^{2}\Bigg] \Psi+\mathcal{O}\lr{\frac{\xi^2}{{\mq^4}}}$}.\label{SpinorLagPert}
\end{align}
where $Q$-induced interactions couple the matter field to the Bumblebee and we have neglected the spinors coupling to torsion as explained above in footnote \ref{foot1Bumb}.

As the Bumblebee field develops a nontrivial VEV, the $Q$-induced interactions with the Bumblebee in the above effective Lagrangians can carry coefficients for Lorentz violation. However, for these coefficients to be observable, they have to be nonvanishing for a stable nontrivial Bumblebee vacuum. Thus, before analysing these coefficients, we must study the vacuum structure of the bumblebee field in search for stable nontrivial VEVs. To that end, we have to specify first a particular form for the Bumblebee potential which provides spontaneous breaking of Lorentz symmetry. We will choose the usual Mexican hat potential, given by
\begin{equation}
V(B^\mu B_\mu\mp b^2)=\frac{\lambda}{4}\big(B^\mu B_\mu\mp b^2\big)^2,
\end{equation}
where $\lambda$ is a positive weak coupling. Here $b^2>0$ and the $\mp$ sign accounts for the possibility of having a spacelike or timelike Bumblebee VEV respectively.  With this choice of potential, the Einstein frame Lagrangian for the Bumblebee reads
\begin{equation}
\resizebox{.9\hsize}{!}{${\cal L}_{BEF}=-\frac{1}{4}B_{\mu\nu}B^{\mu\nu}+\frac{M^2}{2}B^2-\frac{\Lambda}{4}(B^2)^2+\frac{\xi}{{\mq^2}}\Big[B^{\mu\nu}B^\alpha{}_{\nu}B_\mu B_\alpha-\frac{1}{4}B_{\mu\nu}B^{\mu\nu}B^2-\frac{3}{4}\Lambda(B^2)^3\Big]+\mathcal{O}\lr{\frac{\xi^2}{{\mq^4}}}$}\label{BumbLagPert}
\end{equation} 
respectively, where the Bumblebee effective mass is given by
$M^2= \lambda b^2\lr{\pm 1+\frac{\xi}{2{\mq^2}}b^2}$ and $\Lambda\equiv \lambda\lr{1\pm \frac{4\xi}{\mq^2}b^2}$. Given that we are only interested in the qualitative details of the vacuum structure, and we are considering $\xi$ as a perturbative coupling, it will suffice to unveil the vacuum structure in the $\xi\rightarrow0$ limit. In other words, the perturbative modifications introduced by $\xi$ will not change the number and nature of the vacua, so that we can study the vacuum structure of the $\xi\rightarrow0$ case.

\subsection{Stability of the Bumblebee vacua}

The explicitly covariant form of the Bumblebee Lagrangian \eqref{BumbLagPert} is a constrained theory, as $B_0$ is non-dynamical due to the gauge invariant kinetic term (see section \ref{sec:GhostsInCurvatureBased}). Indeed, the corresponding field equations for $B_0$ in the $\xi\to0$ limit are
\begin{equation}
\lambda B_0\left(B_0^2-{\textbf{B}}^2-\frac{\mu}{\lambda}\right)-\partial_i \dot B^i=0,
\end{equation}
where ${\textbf{B}}^2=\delta^{ij}B_iB_j$ and $\mu=\pm M^2$. This is an algebraic equation for $B_0$ and, already for the $\xi\to0$ case, there will be different branches of the theory corresponding to one of the three solutions to the above constraint equation. Since we are doing the analysis perturbatively in $\xi$, we will just be interested in the vacuum structure of the $\xi\to0$ theory, and the stability properties of each of the vacua will not change perturbatively in $\xi$. The above constraint equation has three solutions that can be parametrised in the general form
\begin{equation}\label{B0solutions}
B_0^{(k)}=a_k\frac{\bar{B}}{3 A}+a_k^\ast A
\end{equation}
where
\begin{equation}
\bar{B}\equiv {\textbf{B}}^2+\frac{M^2}{2},\quad A\equiv\left(\frac{\partial_i \dot B^i}{2 \lambda }+\sqrt{\left(\frac{\partial_i \dot B^i}{2 \lambda }\right)^2-\left(\frac{\bar{B}}{3}\right)^3}\right)^{1/3}
\end{equation}
and the three solutions are given by
\begin{equation}
a_1=1,\qquad a_2=-\frac{1+{\textrm{i}}\sqrt{3}}{2} \quad\text{and}\quad a_3=a_2^\ast,
\end{equation}
so that $B_0^{(3)}=B_0^{(2)}{}^\ast$. The only branch admitting a Lorentz invariant vacuum, namely $B_0=0$ and $B_i=0$ is the $B_0^{(1)}$ branch, which admits it for both signs. To see that, take $B_i=0$ (then $\partial_i \dot B^i=0$ too). The values for three branches are
\begin{equation}\label{LIvacuum}
B_0^{(1)}|_{B_i\to 0}=0,\qquad B_0^{(2)}|_{B_i\to 0}\propto B_0^{(3)}|_{B_i\to 0}\propto \sqrt{\frac{|\mu|}{\lambda}},
\end{equation}
the proportionality factors are given by $\pm 1$ for the $+|M^2|$ case and $\pm \mathrm{i}$ for the $-|M^2|$ case. Note however that the fact that the $B^{(0)}$ solution for the constraint is compatible with the trivial configuration for $B_\mu$ does not necessarily imply that this configuration is a (Lorentz invariant) vacuum of the theory. This must be analysed by checking the vacuum structure corresponding to the Lagrangian \eqref{BumbLagPert}, which will allow us to see whether the different branches have Lorentz violating (meta)stable vacua where we can compute the quantum corrections associated to the different fields of the theory. To that end, one has two options: 1) compute the quadratic actions for perturbations to $B_\mu=\beta_\mu+\tilde{B}_\mu$ around any background, then integrate out the non-dynamical $\tilde{B}_0$ by solving the corresponding (linear) constraint equation, and study the eigenvalues of the kinetic matrix for the perturbations $\tilde{B}_i$ on top of each of the vacua, or 2) resort to the Hamiltonian formalism. Let us proceed with 2). To that end, after solving the constraint equation for $B_0$, the Hamiltonian to analyse reads
\begin{align}
H_k=&\frac{1}{2}\vec{E}^2+\frac{1}{4}B_{ij}B^{ij}-\left(a_k \frac{\bar B^2}{3A}+a_k^\ast A\right)\partial_i E^i+\frac{\lambda}{4}\Bigg[a_k \left(\frac{\bar B^2}{3A}\right)^4\nonumber\\
&+a_k^\ast A^4-2 a_k^\ast\left(\frac{\bar B^2}{3}\right)^3\frac{1}{A^2}-a_k\frac{2\bar B^2}{3A} A^2+\frac{(\bar B^2)^2}{3}\Bigg]
\end{align}
where we have dropped a constant term and $\vec{E}^2=\delta^{ij}E_iE_j$, where we have defined 
\begin{equation}
E^i\equiv\left.\frac{\partial\mathcal{L}_{BEF}}{\partial \dot B_i}\right|_{\xi\to 0}
\end{equation}
as the conjugate momenta to $B_i$. The constraint equation is now solved in terms of $B_i$ and the conjugate momenta as in \eqref{B0solutions} with $A$ now given by
\begin{equation}
A\equiv\left(\frac{\partial_i E^i}{2 \lambda }+\sqrt{\left(\frac{\partial_i E^i}{2 \lambda }\right)^2-\left(\frac{\bar{B}}{3}\right)^3}\right)^{1/3}.
\end{equation}

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{Figures/FigPotnegfull.png}
\includegraphics[width=\textwidth]{Figures/FigPotneg0.png}
\caption{\label{FigPotpos} In the upper row we plot the phase space potential for the Bumblebee field as a function $V(\textbf{B},\partial_i E^i)$ for the three $B_0$ branches for the $-|M^2|$ case. The black dot highlights the point $(0,0,V(0,0))$. We can see how only the $B_0^{(1)}$ branch has a critical point for the potential, namely a minimum, which corresponds to the trivial vacuum. This minimum is global within the $B_0^{(0)}$ branch, but it is local if the full solution space is considered, given that the potential is not bounded for below for the other branches $B_0^{(i\neq1)}$. Thus, it corresponds to a classically stable Lorentz invariant vacuum that can decay by quantum tunneling. In the lower row, the same potentials are plotted close to the trivial configuration $\textbf{B}=0$ and $\partial_i E^i=0$. We can appreciate clearly how the $B_0^{(1)}$ branch has a minimum at this point, while the two other branches do not have any critical point there.}
\end{figure*}


Now we must consider the two possible signs for $M^2$, which lead to different vacuum structures. Let us start first with the $-|M^2|$ case.  Here, we see that $\bar B$ is strictly positive for all values of $B_i$, and we can write the Hamiltonian perturbatively for each of the three branches as
\begin{equation}
\begin{split}
H&^{-}_k=\frac{1}{2}\vec{E}^2+\frac{1}{4}B_{ij}B^{ij}+\frac{\lambda}{4}(1-n_{k}^2)\left({\textbf{B}}^2+\frac{|M^2|}{\lambda}\right)^2\\
&+n_k\sqrt{{\textbf{B}}^2+\frac{|M^2|}{\lambda}}\partial_i E^i+\frac{(\partial_i E^i)^2}{2(1-2n_{k}^2)\lambda\left({\textbf{B}}^2+\frac{|M^2|}{\lambda}\right)}
\end{split}
\end{equation}
up to $\mathcal{O}\left((\partial_i E^i)^3\right)$ corrections, where
\begin{equation}
n_1=0,\qquad n_2=1 \quad\text{and}\quad n_3=-1
\end{equation}
characterise each branch. Now, note that the $B_0^{(1)}$ branch does not have a linear term in $\partial_i E^i$, and the quadratic term is positive definite, as are all the remaining ones. The configuration $B_i=0$ and $E^i=0$ is a classically stable vacuum with a value for the Hamiltonian of $M^4/4\lambda$ which, in this branch, is Lorentz-invariant since, $B^{(1)}_0$ is also vanishing for the trivial configuration due to its constraint equation. For the other two branches, this field configuration leads to a vanishing Hamiltonian, so that the $B_i=E^i=0$ vacuum of the $B_0^{(1)}$ branch is a local minimum and, though classically stable, it can decay through tunnelling processes turning it into a metastable vacuum. In figure \ref{FigPotpos} we plot the relevant piece of the full Hamiltonian for each of the branches. As expected, the $B_0^{(1)}$ branch has a classically stable vacuum at $B_i=E^i=0$. However, we see that the $B_0^{(2)}$ and $B_0^{(3)}$ branches do not have any extremal points due to the fact that its derivative in the $\partial_i E^i$ direction never vanishes.\\

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{Figures/FigPotposfull.png}
 \includegraphics[width=\textwidth]{Figures/FigPotpos0.png}
\caption{\label{FigPotneg} In the upper row we plot the phase-space potential for the Bumblebee field as a function $V({\textbf{B}},\partial_i E^i)$ for the three $B_0$ branches in the case $\mu=-M^2<0$. The black dot highlights the point $(0,0,V(0,0))$ in the $B_0^{(1)}$ branch plot and the points $(\pm\sqrt{M^2/\lambda},0,0)$. We can see how in the $B_0^{(1)}$ branch the trivial Lorentz invariant vacuum is unstable, as expected for a tachyonic mass sign. As opposed to the $\mu>0$ case, now there is a pair of (degenerate) nontrivial vacua in the $B_0^{(3)}$ branch which spontaneously breaks Lorentz symmetry spatially, as the Bumblebee condenses to $(0,B_i)$ with ${\textbf{B}}=\sqrt{M^2/\lambda}$. This vacuum is a global minimum within the $B_0^{(3)}$ branch, though the potential is not bounded from below for the other branches $B_0^{(i\neq1)}$, turning it into a pair of metastable Lorentz violating vacua. The potential for the $B_0^{(2)}$ branch does not have any critical points. In the lower row, the same potentials are plotted close to the trivial configuration ${\textbf{B}}=0$ and $\partial_i E^i=0$ to allow for better appreciation of these features.}
\end{figure*}


For the $+|M^2|$ case, the expansion of the Hamiltonian around the trivial configuration reads
\begin{equation}
\begin{split}
H&^{+}_k=\frac{1}{2}\vec{E}^2+\frac{1}{4}B_{ij}B^{ij}+\frac{\lambda}{4}(1-n_{k}^2)\left({\textbf{B}}^2-\frac{|M^2|}{\lambda}\right)^2\\
&- n_k\,{\textrm{i} }\sqrt{-{\textbf{B}}^2+\frac{|M^2|}{\lambda}}\partial_i E^i+\frac{(\partial_i E^i)^2}{2(1-2n_{k}^2)\lambda\left({\textbf{B}}^2-\frac{|M^2|}{\lambda}\right)}
\end{split}
\end{equation}

which has an imaginary coefficient for the linear term in the $B^{(2)}_0$ and $B^{(3)}_0$ branches if $\textbf{B}^2<|M^2|/\lambda$. Thus we have to analyse the full Hamiltonian for (at least) these branches. Indeed, though the above expansion of the Hamiltonian is real around the trivial configuration for the $B^{(1)}_0$ branch, this is an artefact of the expansion, and higher order terms become complex around the trivial configuration except in the $\partial_iE^i=0$ direction, as can be seen in figures \ref{FigPotpos} and \ref{DerPotZero}. We thus have to proceed with the analysis of the full Hamiltonian for the $+|M^2|$ case. In figure \ref{FigPotpos} we plot the relevant piece of the Hamiltonian to analyse the vacuum structure of each of the branches. We see that, unlike expected from the perturbative expansion, the $B^{(3)}_0$ branch leads to a real Hamiltonian around the trivial configuration $B_i=E^i=0$, where it has a temporally broken unstable vacuum with $B_0=\sqrt{|M^2|/\lambda}$. The $B^{(2)}_0$ is complex around $B_i=E^i=0$, and its only vacua is a saddle point at $\textbf{B}^2=|M|/\sqrt{\lambda}$ and $\partial_i E^i=0$, which is also present in the $B^{(3)}_0$ branch. The behavior of the $B^{(1)}_0$ branch is surprising due to the fact that it becomes complex for
\begin{equation}
\left(\frac{\partial_i E^i}{2 \lambda}\right)^2-\left(\textbf{B}^2-\frac{|M^2|}{\lambda}\right)^3>0,
\end{equation}
which is solved by
\begin{equation}
|\textbf{B}|>\sqrt{3\left(\frac{\partial_i E^i}{2 \lambda}\right)^{2/3}+\frac{M^2}{\lambda }},
\end{equation}
except in the $\partial_i E^i=0$ direction, where it is constant and equal to zero from $\textbf{B}^2=|M^2|/\lambda$ up to $\textbf{B}^2=0$. This can be verified by plotting the directional derivative of the (relevant part of the) Hamiltonian in the $\textbf{B}$ direction for fixed values of $\partial_i E^i$, as done in figure \ref{DerPotZero}. In figures \ref{FigPotpos} and \ref{DerPotZero}, we see that for $\partial_i E^i=0$, there is a continuum and degenerated set of minima defined by $\textbf{B}^2\in(|M^2|/\lambda,0)$ which break Lorentz symmetry except for the trivial one. We can also see that for other branches the Hamiltonian is not bounded from below so, although these degenerated vacua are classically stable, thecan also decay through quantum tuneling, being thus metastable Lorentz-breaking vacua.

To sum up, we see that for the $-|M^2|$ case, the only classically stable vacuum is the trivial one. On the other hand, for the $+|M^2|$ case, there is a degenerate set of local minima which corresponds to metastable Lorentz breaking vacua characterised by $\partial_i E^i=0$ and $\textbf{B}^2\in(|M^2|/\lambda,0)$. As a remark, let us comment that, though everything seems to indicate that there is a continuum of Lorentz-breaking metastable vacua connected to the trivial one in the $+|M^2|$ case, in agreement with previous literature on the Bumblebee model (see e.g. \cite{Bluhm:2008yt}), the regions where the Hamiltonian becomes complex deserve a more detailed analysis to better understand their properties.\\

\begin{figure*}[h]
\centering
\includegraphics[width=0.45\textwidth]{Figures/FigHamBidirectiondE0.png}
\includegraphics[width=0.45\textwidth]{Figures/FigDerHamBidirectiondE0.png}
\caption{\label{DerPotZero} Here we plot the phase space potential for a fixed value $\partial_i E^i=0$ for the $B^{(1)}_0$ branch and for the two choices in $\pm|M^2|$ as well as for a vanishing mass. There, it can be seen how, despite developing a complex part for any $\partial_i E^i>0$ if $\textbf{B}^2$ is small enough, the Hamiltonian is real for any value of $\textbf{B}^2$ if $\partial_i E^i$ is fixed to zero. We can also see how the directional derivative in the $\textbf{B}$ direction vanishes from $\textbf{B}^2=|M^2|/\lambda$ up to $\textbf{B}^2=0$, showing a continuous set of (classically stable) Lorentz breaking vacua characterised by from $\textbf{B}^2\in(M^2|/\lambda,0)$ and $\partial_i E^i=0$.}
\end{figure*}

\section{Lorentz-violating coefficients}

We now know that there is a classically stable nontrivial timelike vacuum for the bumblebee field in the $\mu<0$ case. We will first consider an approximately\footnote{In presence of a nontrivial gravitational field, this condition is not well defined, but we are neglecting those effects.} constant timelike VEV  $\langle B_\mu\rangle=b_\mu=(0,b_i)$ with $\delta^{ij}b_i b_j=b^2=M^2/\lambda$ in a weak gravitational field. Later we will generalise for arbitrary timelike VEVs. Generally, observables which couple to $b_{\mu}$ will be sensitive to the spontaneous breaking of Lorentz symmetry by the Bumblebee field. Since the present model displays non-minimal couplings between the Bumblebee field and the matter sources through the non-Riemannian part of the connection, there will arise several Lorentz violating (LV) coefficients in the Einstein frame effective matter sector. 
 
\subsubsection{Scalar field}
The Lagrangian for a scalar field propagating on top of the nontrivial Bumblebee background  takes the form
\begin{eqnarray}
\nonumber\mathcal{L}_{sc}&=&-\frac{1}{2}\Phi(\Box+m^2)\Phi+\frac{\xi}{{\mq^2}}\Phi\Big[(s^{\mu\nu}\partial_{\mu}\partial_{\nu})+\frac{1}{2}m^2 b^2\Big]\Phi+\mathcal{O}\lr{\frac{\xi^2}{{\mq^4}}},\label{ScalarLagBackground}
\end{eqnarray}
where $s^{\mu\nu}= b^{\mu}b^{\nu}$. The $\mathcal{O}(\xi)$ terms will typically induce LV coefficients through the VEV of the Bumblebee field. The $s^{\mu\nu}$ term constitutes a modification of the standard kinetic term which can be encoded in an effective metric for the scalar field of the form $g_{\textrm{eff}}^{\mu\nu}=\eta^{\mu\nu}-(2\xi/{\mq^2}) s^{\mu\nu}$ for a generic background. However, in the classically stable background, $s^{00}=s^{0i}=0$, which modifies only the coupling with the spacial derivatives. Hence, a ``wrong'' signature of the LV coefficient $s^{\mu\nu}$ could trigger Laplacian instabilities around strong enough Bumblebee backgrounds (see chapter \ref{sec:UnstableDOF}). Note, however, that in such case, the perturbative expansion would break down given that $(\xi/{\mq^2}) b^2$ would be $\mathcal{O}(1)$, and a full non-perturbative analysis would be required. The correction to the mass term in (\ref{31}) can also be encoded in an effective mass of the form $m_{\textrm{eff}}^2=m^2(1-(\xi/{\mq^2}) b^2)$ which could also trigger tachyonic-like instabilities for a space-like Bumblebee VEV (again non-perturbative effects could play a non-negligible role). 

In order to explore potential instabilities in more detail, let us analyse the dispersion relation of the classically stable vacuum, which reads
\begin{equation}\label{disprelscalarspacelike}
E^2=\vec{p}^2+m^2+\frac{2\xi}{\mq^2} \left(\frac{1}{2} m^2 b^2+(\vec{b}\cdot\vec{p})^2\right) +\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}}.
\end{equation}
This dispersion relation is healthy for positive values of $\xi$. For negative values of $\xi$ a tachyonic-like instability as well as a Laplacian instability  (in directions which are non-orthogonal to $\vec{b}$) could potentially arise. In case that these instabilities appear, we should check their persistence in a full nonperturbative analysis of the theory.

\subsubsection{Dirac field}

Let us now turn our attention to the spin $1/2$ fields. To explore the physics of our interest in a more convenient way, we will work with the decomposition of LV coefficients that is more commonly used in the literature \cite{Colladay:1996iz,Colladay:1998fq}. To that end, let us write the weak-field spinor action on top of a nontrivial Bumblebee background as \eqref{SpinorLagPert} as 
 \begin{equation}
\mathcal{L}_{sp}=\bar{\Psi}\left(i\Gamma^{\mu}\partial_{\mu}- \hat M\right)\Psi,
\label{SpinorLagShort}
\end{equation}
where ${\Gamma}^{\mu}$ and ${M}$ are elements of the 16-dimensional Clifford algebra defined by the Dirac gamma matrices. We can thus expand them in the usual basis of this algebra as
\begin{equation}
\begin{split}
{\Gamma}^{\mu}&={e}^{\mu}I+(\delta^\mu{}_\alpha+{c}^{\mu}{}_{\alpha})\gamma^{\alpha}+{d}^{\mu}{}_{\alpha}\gamma_{5}\gamma^{\alpha}+i{f}^{\mu}\gamma_{5}+\frac{1}{2}{g}^{\mu}{}_{\lambda\alpha}\sigma^{\lambda\alpha},\\
{\hat M}&={m}_{\textrm{eff}}I+{a}_{\mu}\gamma^{\mu}+{k}_{\mu}\gamma^{\mu}\gamma_{5}+\frac{1}{2}l_{\mu\nu}\sigma^{\mu\nu},
\label{LVSpinorDecomp}
\end{split}
\end{equation} 
where ${c}^{\mu}{}_{\alpha}$, ${d}^{\mu}{}_{\alpha}$, ${e}^{\mu}$, ${f}^{\mu}$, ${g}^{\mu}{}_{\lambda\alpha}$, ${a}_{\mu}$, ${k}_{\mu}$ and $l_{\mu\nu}$ are LV coefficients. Comparing \eqref{SpinorLagPert} to \eqref{SpinorLagShort} and \eqref{LVSpinorDecomp}, we find the non-zero LV coefficients
\begin{eqnarray}
{c}^{\mu}{}_{\alpha}&=&\frac{\xi}{{2\mq^2}}\lr{\frac{M^2}{\lambda}\delta^{\mu}{}_\alpha+2b^\mu b_\alpha}+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},\\
{m}_{\textrm{eff}}&=&m\left(1+\frac{\xi}{{\mq^2}} \frac{M^2}{\lambda}\right)+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}}.
\label{coeff}
\end{eqnarray}
We see that within the metric-affine Bumblebee model, the LV coefficients that appear provide a modification of the fermionic mass through $m_{\textrm{eff}}$ {and} a modification of the standard kinetic term through ${c}^{\mu}_{}{\alpha}$. In general, these will introduce modifications in the dispersion relation of spin $1/2$ fields. To find them let us write the Dirac equation derived from \eqref{SpinorLagShort} as
 \begin{equation}\label{SpinorEqShort}
\left(i\Gamma^{\mu}\partial_{\mu}- \hat M\right)\Psi=0\ , 
\end{equation}
 and multiplying on the left by $\left(i\Gamma^{\mu}\partial_{\mu}+M\right)$ we arrive at
\begin{align}
\begin{split}
\lrsq{\Gamma^\mu\Gamma^\nu\partial_{\mu}\partial_{\nu}-i[\hat M,\Gamma^\mu]\partial_{\mu}+\hat M^2} \Psi=0 \ .
\end{split}
\end{align} 
By using now the relations
\begin{align}
&\{\Gamma^\mu,\Gamma^\nu\}=2\eta^{\mu\nu}+\frac{2\xi}{{\mq^2}}\lr{\frac{M^2}{\lambda}\eta^{\mu\nu}-2b^\mu b^\nu}+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},\\
&[ \hat M,\Gamma^\mu]=\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},\\
& \hat M^2=m^2\left(1+\frac{2\xi}{{\mq^2}} \frac{M^2}{\lambda}\right)+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},
\end{align}
we find the following dispersion relation
\begin{align}
%\begin{split}
\nonumber&\lrsq{E^{2}\lr{1+\frac{2\xi}{{\mq^2}}\frac{M^2}{\lambda}}-\left(1+\frac{2\xi}{{\mq^2}} \frac{M^2}{\lambda}\right)\left(\vec{p}^{2}+m^{2}\right)-\frac{2\xi}{{\mq^2}}(\vec{p} \cdot \vec{b})^{2}} \Psi=\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}} \ .
%\end{split}
\end{align}
For a (constant) spacelike VEV $b_{\mu}=[0,\vec{b}]$ we obtain
\begin{eqnarray}
E^{2}=\vec{p}^2+m^2+\frac{2\xi}{{\mq^2}} (\vec{p}\cdot\vec{b})^2+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}} \ .
\end{eqnarray}
For any sign of $\xi$, the $\cO(\xi)$ term could trigger Laplacian instabilities at the perturbative level, though a full analysis should be carried out in order to check that the instabilities are not an artefact of the perturbative expansion. See \cite{Kostelecky:2000mm} for a discussion on the typical energy scales at which these instabilities become relevant. Available constraints on LV parameters, as well as on the characteristic scale of instabilities if these are developed, could be used to constrain the allowed values of the nonminimal coupling sourcing LV in the matter sector.

\subsubsection{Arbitrarily varying $b_\mu$}
\label{app1}
If we drop the assumption of constant $b_\mu$, we find the effective Lagrangian for scalar fields
\begin{eqnarray}
\nonumber\mathcal{L}_{sc}=-\frac{1}{2}\Phi(\Box+m^2)\Phi+\frac{\xi}{{\mq^2}}\Phi\Big[(s^{\mu\nu}\partial_{\mu}\partial_{\nu})+ t^\mu \partial_\mu-\frac{M^2}{2\lambda}m^2 \Big]\Phi+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},
\end{eqnarray}
with $t^\mu=b^\mu(\partial_\nu b^\nu)+b^\nu(\partial_\nu b^\mu)$. Note  the presence of the additional coefficient $t_\mu$ in relation to the standard case (it vanishes for constant Bumblebee VEVs). This coefficient introduces an imaginary term in the scalar dispersion relation. The modified scalar dispersion relations now looks
\begin{align}
\nonumber&E^2 -\vec{p}^2-\lrsq{1-\frac{\xi}{{\mq^2}}\frac{M^2}{\lambda}}m^2-\frac{2\xi}{{\mq^2}} (\vec{b}\cdot\vec{p})^2+\frac{2\xi}{{\mq^2}}(-\vec{b}+i\vec{t})\cdot\vec{p} =\mathcal{O}\lr{\frac{\xi^2}{\mq^2}}.\label{disprelscalar}
\end{align}
Note the existence of imaginary terms in the above dispersion relation, which only vanish if  one considers a frame where $t^{\mu}p_{\mu}=0$. This undesired property leads to complex eigenvalues of the Hamiltonian operator,  which  turns out to be non-Hermitian, and potential Laplacian instabilities.   

For spinor fields, the dispersion relation is modified in relation to the constant $b_{\mu}$ as 
\begin{align}
\big(\Gamma^\mu\Gamma^\nu\partial_{\mu}\partial_{\nu}+\Gamma^{\mu}(\partial_{\mu}\Gamma^{\nu})\partial_{\nu}+i\Gamma^{\mu}\partial_{\mu}\hat M-i[\hat M,\Gamma^\mu]\partial_{\mu}+M^2\big) \Psi=0.
\end{align} 
Now the relevant relations are
\begin{align}
&\{\Gamma^\mu,\Gamma^\nu\}=2\eta^{\mu\nu}+\frac{2\xi}{{\mq^2}}\lr{\frac{M^2}{\lambda}\eta^{\mu\nu}+2b^\mu b^\nu}+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},\\
&[ M,\Gamma^\mu]=\frac{i}{2} a_\alpha \sigma^{\alpha\mu}+\mathcal{O}\lr{\frac{2\xi^2}{\mq^2}},\\
& M^2=m^2\left(1-\frac{2\xi}{{\mq^2}} b^2\right)+2m  a_\mu \gamma^\mu+\mathcal{O}.\lr{\frac{2\xi^2}{\mq^2}},
\end{align}
We find the following dispersion relation
\begin{eqnarray}
&E^{2}\lr{1+\frac{2\xi}{{\mq^2}} \frac{M^2}{\lambda}}+ \frac{2\xi}{{\mq^2}}E \lr{\frac{i}{2} a_i \sigma^{i 0}-i\gamma^{\mu}\gamma^{\beta}\partial_{\mu}c_{0\beta}}-\left(1-\frac{2\xi}{{\mq2}} \frac{M^2}{\lambda}\right)\left(\vec{p}^{2}+m^{2}\right)\\
&+\frac{2\xi}{{\mq^2}}\lr{-(\vec{p} \cdot \vec{b})^{2}+i\gamma^{\mu}\gamma^{\alpha}\partial_{\mu}a_{\alpha}+\frac{i}{2} a_\alpha \sigma^{\alpha i} p_i-2m a_\mu \gamma^\mu}=\nonumber \mathcal{O}\lr{\frac{2\xi^2}{\mq^2}}.
\end{eqnarray}
Although we can see in the form of the terms that Laplacian instabilities could arise, the analysis of the instabilities in this case appears more intricate than in the constant one. However, we conclude that a non-constant $b_{\mu}$ produces an effective Minkowskian theory which will in general present instability issues.


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

			%NEWCHAPTER%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{A scale invariant notion of time in presence of arbitrary nonmetricity}\label{sec:GeneralisedTime}

\section{Introduction}

From a geometrical perspective, the torsion tensor measures the failure to close for infinitesimal loops built by parallel transport,  while the nonmetricity tensor measures how parallel transport modifies lengths and angles. Concretely, if we decompose the nonmetricity into its irreducible components, its Weyl component controls the change in length of a parallely transported vector. spacetimes where the nonmetricity is fully specified by its Weyl component are named Weyl spacetimes, honoring the first work where this kind of nonmetricity was taken into account by Weyl \cite{Weyl:1918ib}. This irreducible component of the nonmetricity tensor transforms as a gauge 1-form under scale transformations of the metric, {\it i.e.,} it is the gauge field associated to scale transformations (usually called dilaton field). This fact fostered the interest in Weyl geometries, since they provide a natural way of introducing scale transformations without changing the affine structure (which cannot be done in Riemannian geometries). However, though a Weyl-like nonmetricity is necessary for defining scale transformations that do not change the affine structure, the usual restriction on the nonmetricity to be of this form in conformal invariant theories is unnecessary, and this can be achieved with general nonmetricity \cite{Delhom:2019yeo}. In this case only the vectorial irreducible components of nonmetricity transform as a gauge 1-form, while the tensorial irreducible components transform trivially by a conformal factor\footnote{Concretely under a conformal transformation  $g\mapsto\tilde g=e^\phi g$ in 4 spacetime dimensions, the different irreducible components listed in \eqref{decompNM} transform as: $\tilde Q_{1\mu}=Q_{1\mu}+4 (d\phi)_\mu$ , $\tilde Q_{2\mu}=Q_{1\mu}+ (d\phi)_\mu$, $\tilde S_{\mu\al\be}=e^\phi S_{\mu\al\be}$ and $M_{\mu\al\be}=e^\phi M_{\mu\al\be}$}.

 Motivated by the discussion of Perlick  \cite{PerlickTime} about how to construct a suitable Weyl-invariant notion of proper time that reduces to the standard definition of proper time in the Riemannian limit, and following  \cite{Lobo:2018zrz} in its analysis of the physical role played by the Weyl 1-form, in this chapter we will be concerned about finding a suitable definition of proper time that respects scale invariance in the presence of arbitrary nonmetricity (or generalised Weyl invariance in the sense of \cite{Delhom:2019yeo}), and also with the physical consequences of having nontrivial nonmetricity if there were physical clocks which were sensitive to this notion of time. To that end we will generalise the parametrisation for generalised proper time (GPT) found in \cite{Avalos:2016unj} to the case of arbitrary nonmetricity and find the existence of a conformally invariant second clock effect related to Weyl component of the nonmetricity tensor. We will then discuss GPT in light of the  M\"arkze-Wheeler construction (see \eg \cite{MarzkeWheeler,Desloge1989-DESATD,Pauri:2000cr}), which allows to operationally define the notion of clock in GR, elaborating on what kind of matter fields shall one need to build a generalised clock by means of this construction. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalised proper time}\label{sec:GenTime}

The fact that the usual Riemannian proper time, which is defined as the arclength of timelike curves, is not invariant under scale (or Weyl) transformations might be uncomfortable for those who expect UV physics to be scale invariant. To solve this issue, Perlick found a canonical\footnote{Canonical here meaning that uses only the ingredients available in a Weyl structure, or Weyl spacetime.} Weyl-invariant notion of proper time in a Weyl spacetime which reduces to the standard Riemannian proper time in the appropriate limit \cite{PerlickTime}. We will call this Perlick time. Recently, it was shown \cite{Avalos:2016unj} that GPT coincides with the operational time given by Ehlers, Pirani and Schild in \cite{EPS}, where they deduced from an operational point of view, and under certain assumptions regarding freely falling trajectories, that the spacetime manifold could be described by a Weyl spacetime. In \cite{Avalos:2016unj} it was shown that the Perlick time interval between two events $\ga(t_0)$ and $\ga(t)$ belonging to a timelike curve $\ga: t\in I\subset\bbr \mapsto \ga(t)\in \cm$ is given by
\begin{align}\label{PerlickTimeEq} 
\Delta\tau(t)= \frac{\left.\frac{d\tau}{dt}\right|_{(t=t_0)}}{\sqrt{g\lr{\dot\ga(t_0),\dot\ga(t_0)}}}\int_{t_0}^t ds \sqrt{g\lr{\dot\ga(u),\dot\ga(u)}}e^{-\frac{1}{2}\int_{u_0}^u  du \;\om\lr{\dot\ga(u)}} \;,
\end{align}
where $\dot\ga=d\ga (t)/dt$, and in a Weyl space the nonmetricity tensor is given by $\na g=\om\otimes g$. Our aim is to generalise this notion giving a definition of proper time in scale-invariant spacetimes with a general form of the nonmetricity tensor $Q$, {\it i.e.}, in generalised Weyl spacetimes in the sense of \cite{Delhom:2019yeo}. To do so, let us give the definition of Perlick time presented in \cite{PerlickTime}.

A $\tau$-parametrised timelike curve $\ga: \tau\in I \mapsto \ga(\tau)\in M$ is a \textbf{generalised clock} if
\beq\label{DefGenTime}
g\lr{\dot\ga,\nabla_{\dot\ga}\dot\ga}=0 \quad \forall\tau\in I.
\eeq
The parameter $\tau$ parametrising a generalised clock is the \textbf{generalised proper time} (GPT) measured by the clock. It can be shown that every timelike path\footnote{Note that the causal character of a path does not depend on the parametrisation that one uses to describe it as a curve.} $\ga$ admits a parametrisation with GPT \cite{Avalos:2016unj}. In their argument the authors start with a timelike curve $\ga(t)$ and show that a reparametrisation $\mu : t \in I \mapsto \mu(t)=\tau\in I'$ satisfying

\beq\label{ConditionRepClock}
\frac{d^2\mu}{dt^2}-\frac{g\lr{\dot\ga(t),\nabla_{\dot\ga}\dot\ga}}{g\lr{\dot\ga(t),\dot\ga(t)}}\frac{d\mu}{dt}=0
\eeq
has the property that $\tilde{\ga}(\tau)=\ga\circ\mu^{-1}(\tau)$ is a generalised clock. As \eqref{ConditionRepClock} always has a unique solution for timelike paths, every observer can be a generalised clock. The proof outlined in \cite{Avalos:2016unj} is independent of the relation between the metric and affine structure of the spacetime, which allows us to use their result and follow the steps of \cite{Avalos:2016unj} to find a general solution for \eqref{ConditionRepClock} in a spacetime with arbitrary $Q$. In order to derive this solution, let us start from the identity
\beq\label{CompatibiltyCondition}
\lr{\na_X g}(Y,Z)= X\lr{g\lr{Y,Z}}-g\lr{\na_X Y,Z}-g\lr{Y,\na_XZ},
\eeq
where $X,\, Y,\, Z$ are three arbitrary vector fields. Notice that by definition of the nonmetricity tensor, $Q\lr{X,Y,Z}\equiv\lr{\na_X g}(Y,Z)$. Using \eqref{CompatibiltyCondition} with $X=Y=Z=\dot\ga(t)$ and dividing by the tangent vetor squared we find
\beq
\frac{g\lr{\dot\ga,\na_{\dot\ga}\dot\ga}}{g\lr{\dot\ga,\dot\ga}}=\frac{1}{2}\lr{\dot\ga\left[ \ln\lr{g\lr{\dot\ga,\dot\ga}}\right]-\frac{Q\lr{\dot\ga,\dot\ga,\dot\ga}}{g\lr{\dot\ga,\dot\ga}}}\:,
\eeq
which is analogous to Eq.(9) of \cite{Avalos:2016unj} after the substitution\footnote{Notice that this substitution is a particularization of a general nonmetricity tensor to a Weyl-type nonmetricity tensor.} $Q(\dot\ga,\dot\ga,\dot\ga)\mapsto \om\lr{\dot\ga}g\lr{\dot\ga,\dot\ga}$ and taking into account that their $d/dt$ is a derivative in the direction of the curve, so that on a scalar function it is the action of $\dot\gamma$ on that scalar function. Combining this equation with \eqref{ConditionRepClock} yields the following condition for a reparametrisation to lead to a GPT parametrisation in presence of arbitrary nonmetricity
\beq\label{cond_add}
\frac{d\mu}{dt}=\frac{d\mu(t_0)}{dt}\left[\frac{g(\dot\gamma(t),\dot\gamma(t))}{g(\dot\gamma(t_0),\dot\gamma(t_0))}\right]^{1/2}e^{-\frac{1}{2}\int_{t_0}^t ds \frac{Q(\dot\gamma(s),\dot\gamma(s),\dot\gamma(s))}{g(\dot\gamma(s),\dot\gamma(s))}}.
\eeq
Integrating this equation for $\mu=\tau$ leads to an operational expression for computing the GPT elapsed between two events $A=\ga(t_0)$ and $B=\ga(t)$ for the observer $\ga(t)$ in spacetimes with general nonmetricity. This expression reads
\beq\label{GeneralProperTimeEq}
\Delta\tau(t)=\frac{\left.\frac{d\tau}{dt}\right|_{t=t_0}}du{\sqrt{g\lr{\dot\ga(t_0),\dot\ga(t_0)}}}\int_{t_0}^t ds\sqrt{g\lr{\dot\ga(u),\dot\ga(u)}}e^{-\frac{1}{2}\int_{u_0}^u\frac{Q\lr{\dot\ga(s),\dot\ga(s),\dot\ga(s)}}{g\lr{\dot\ga(s),\dot\ga(s)}}},
\eeq
and reduces to the one found for Perlick time \eqref{PerlickTimeEq} if the nonmetricity tensor is specified to be of the Weyl kind. 

A desirable feature for a notion of time is additivity, namely, that the time passed in going from event $A$ to event $B$ through a path $\ga_{AB}$ added to the time passed in going from event $B$ to event $C$ through a path $\ga_{BC}$ is the same as the time passed in going from event $A$ to event $C$ through the path $\ga_{AB}+\ga_{BC}$ where the sum here must be understood as concatenation of paths. The proof of the additivity of GPT in Weyl spacetimes given in \cite{Avalos:2016unj} also works in presence of general nonmetricity, and therefore the additivity is guaranteed. Moreover, due to the fact that \eqref{GeneralProperTimeEq} reduces to \eqref{PerlickTimeEq} for Weyl nonmetricity and, as proven in \cite{Avalos:2016unj}, \eqref{PerlickTimeEq} has the correct Weyl-Integrable-spacetime (WIST) and Riemannian limits, GPT will also have the correct WIST and Riemannian limits, thus being a sensible generalisation of Riemannian proper time in presence of arbitrary nonmetricity.
\par
In post-Riemannian manifolds, the scale invariance of the affine structure implies that the nonmetricity tensor must transform in a particular way under scale transformations. In fact, one can verify that the simultaneous transformations
\begin{equation}\label{conf-trans}
\tilde{\boldsymbol{g}}=e^{\phi}\boldsymbol{g} \ \ \ \ \text{and} \ \ \ \ \tilde{Q}=e^{\phi}(Q+\boldsymbol{d}\phi\otimes \boldsymbol{g})
\end{equation}
leave invariant the affine connection (as scale transformations should), where $\phi$ is any arbitrary smooth scalar function \cite{Delhom:2019yeo}. Since conformal transformations do not modify the orthogonality conditions, from its definition (\ref{DefGenTime}), GPT is scale invariant independently of the affine structure. This can also be verified by using \eqref{conf-trans} on the operational expression \eqref{GeneralProperTimeEq} that allows to explicitly compute the GPT within a given timelike path. Hence GPT is a sensible conformal invariant notion of time not only in Weyl spacetimes, but also in spacetimes with arbitrary nonmetricity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Relation between GPT and Ehlers-Pirani-Schild proper time}\label{sec:EPS}

In the framework introduced by Ehlers, Pirani and Schild (EPS) in \cite{EPS}, one of the key assumptions that lead to the conclusion that the universe should be a Weyl spacetime\footnote{Note that from the metric-affine point of view, a Riemannian spacetime is a particular instance of a Weyl space with $\om=0$. However, the canonical affine structure of a Riemannian spacetime is not conformal invariant.} was the compatibility between the projective structure defined by the trajectories of freely falling particles and the conformal structure defined by the trajectories of light rays. They also define a notion of proper time within this framework which is Weyl invariant and coincides with GPT in Weyl spaces \cite{Avalos:2016unj}. In other words, under the restriction to the nonmetricity tensor of being Weyl-like, the GPT boils down to EPS proper time. In the following, we will be concerned with finding the most general kind of nonmetricity such that equivalence between EPS and GPT holds. To that end, we will proceed by following the proof given in \cite{Avalos:2016unj} for the equivalence of EPS and Perlick clocks but leaving nonmetricity completely arbitrary.

By definition \cite{EPS}, a timelike curve $\ga(\tau)$ is an \textbf{EPS clock}, {\it i.e.}, it is parametrised by \textbf{EPS time}, if there exists a vector field $V_\ga$ parallel along $\ga(\tau)$ which satisfies 
\beq\label{EPSclockDef}
g(\dot\ga(\tau),\dot\ga(\tau))=g(V_\ga(\tau),V_\ga(\tau))
\eeq
along the curve. Differentiating this condition and using that $V_\ga(\tau)$ is parallelly transported along $\ga(\tau)$, namely  $\na_{\dot\ga}V_\ga(\tau)=0$, the following relation follows from \eqref{CompatibiltyCondition}
\begin{align}\label{ConditionEPSisPerlick}
2g\lr{\na_{\dot\ga}V_\ga,\dot\ga}=Q(\dot\ga,V_\ga,V_\ga)-Q(\dot\ga,\dot\ga,\dot\ga)
\end{align}
where al the quantities are evaluated at a point $\ga(\tau)$. This condition is valid for any EPS clock in presence of arbitrary nonmetricity. Hence, by definition of generalised clock \eqref{DefGenTime}, for any EPS clock to be also a generalised clock, the condition 
\beq
Q(\dot\ga,\dot\ga,\dot\ga)=Q(\dot\ga,V_\ga,V_\ga),
\eeq
must be satisfied along any timelike curve $\ga(\tau)$, where $V_\ga(\tau)$ is the vector field satisfying the EPS clock condition \eqref{EPSclockDef} along $\ga(\tau)$. 

Let us now try to answer the opposite question, namely, under which conditions any generalised clock is an EPS clock. By definition, a timelike curve $\ga(\tau)$ is a generalised clock if $\dot\ga(\tau)$ and $\na_{\dot\ga}\dot\ga$ are orthogonal along the curve. Define (locally) a parallel vector field $V_\ga$ along $\ga(\tau)$ as the unique solution to the the initial value problem
\beq\label{InitialValueProblem}
\na_{\dot\ga}V_\ga=0\qquad\text{with initial condition}\qquad V_\ga(\tau_0)=\dot\ga(\tau_0).
\eeq
Using parallelism of $V_\ga$ along $\ga(\tau)$ and the orthogonality between $\dot\ga(\tau)$ and $\na_{\dot\ga}\ga$, subtracting \eqref{CompatibiltyCondition} applied to $X=\dot\gamma$ and $Y,Z=V_\ga,\dot\ga$, one finds that the initial value problem
\begin{align}
\frac{d}{d\tau}\Big(g\lr{V_\ga,V_\ga}-g\lr{\dot\ga,\dot\ga}\Big)=Q(\dot\ga,V_\ga,V_\ga)-Q(\dot\ga,\dot\ga,\dot\ga)\quad\text{with }\quad V_\ga(\tau_0)=\dot\ga(\tau_0)
\end{align}
must be solved along $\ga(\tau)$. The initial condition guarantees the vanishing of both sizes at $\tau=\tau_0$. Thus, given the form of the above initial value problem, and the uniqueness of its solution, the initial condition will remain true along $\ga(\tau)$, and therefore any EPS clock $\ga(\tau)$ will also be a generalised clock, if and only if
\beq\label{ConditionPerlickisEPS}
Q(\dot\ga,V_\ga,V_\ga)=Q(\dot\ga,\dot\ga,\dot\ga)
\eeq
is satisfied along any timelike curve $\ga(\tau)$. Therefore, the condition \eqref{ConditionPerlickisEPS} is a necessary and sufficient condition for any generalised clock to be an EPS clock. 

The natural next step is to find out what is the most general kind of nonmetricity tensor that satisfies the above condition. To that end, let us proceed as follows. For every timelike curve $\ga(\tau)$, define a symmetric  (0,2) tensor by $q^{(\ga)}=\na_{\dot\ga} g$. With this definition, and given an atlas covering $\gamma$, the condition \eqref{ConditionPerlickisEPS} can be written as 
\begin{equation}\label{CondQEPS=Perlick}
q^{(\ga)}{}_{\al\be}\lr{V_{\ga}{}^\al V_{\ga}{}^\be-\dot\ga^\al\dot\ga^\be}=0,
\end{equation}
which has to be satisfied for all timelike paths for some parametrisation. The above condition gives only one algebraic constraint given by \eqref{ConditionPerlickisEPS} for 10 independent components of $q^{(\ga)}{}_{\al\be}$. Thus the system is indeterminate, which makes sense, given that we know that any Weyl spacetime satisfies this condition. However, let us try to solve the system step by step to confirm this. Since it is homogeneous, there is the trivial solution $q^{(\ga)}=0$ for all $\ga(\tau)$ which implies that the nonmetricity must vanish, \ie a Riemannian spacetime is a particular case of spacetimes where EPS and generalised clock coincide. There is another solution that can be found by looking at the definition of an EPS clock \eqref{EPSclockDef}. From that definition, it is  apparent that for any spacetime that satisfies ${q}^{(\ga)}=\phi_\ga g$ where $\phi_\ga$ is an arbitrary scalar function that depends on the particular path. If that is the case, at each point $p\in\cm$, we can define a 1-form $\omega\in\ctb$ such that $\omega_{p}[\dot\gamma_p]=\phi_\ga(p)$ for each timelike path through $p$, so that for any pair of vectors fields $A,B$ and timelike path parametrised by $\ga(\tau)$ we have
\beq
q^{(\gamma)}(A,B)=\omega[\dot\gamma]g(A,B), 
\eeq
which implies that $Q=\omega\otimes g$, \ie all Weyl spacetimes are a solution to the above system as expected.
In order to see whether there are any other solutions to the system, we can look at the above conditions when written in terms of the irreducible components of the nonmetricity tensor. In 4 spacetime dimensions, the nonmetricity tensor can be decomposed in its Lorentz-irreducible pieces as
\begin{align}\label{NMdecomposed}
\resizebox{0.9\hsize}{!}{$Q_{\mu\alpha\beta}=\frac{1}{18}(5Q_{1\mu} g_{\alpha\beta}-Q_{1\alpha} g_{\beta\mu}-Q_{1\beta} g_{\mu\alpha}-2Q_{2\mu} g_{\alpha\beta}+4Q_{2\alpha} g_{\beta\mu}+4Q_{2\beta} g_{\mu\alpha})+S_{\mu\alpha\beta}+M_{\mu\alpha\beta},$}
\end{align}
where the different objects are
\begin{align}
\begin{split}\label{decompNM}
&Q_{1\mu}\equiv  g^{\alpha\beta}Q_{\mu\alpha\beta} \ \ \  , \ \ \ Q_{2\mu}\equiv  g^{\alpha\beta}Q_{\alpha\mu\beta},\\
&\resizebox{0.9\hsize}{!}{$S_{\mu\alpha\beta}\equiv \frac{1}{3}(Q_{\mu\alpha\beta}+Q_{\alpha\beta\mu}+Q_{\beta\mu\alpha})-\frac{1}{18}(Q_{1\mu} g_{\alpha\beta}+Q_{1\alpha} g_{\beta\mu}+Q_{1\beta} g_{\mu\alpha})-\frac{1}{9}(Q_{2\mu} g_{\alpha\beta}+Q_{2\alpha} g_{\beta\mu}+Q_{2\beta} g_{\mu\alpha})$},\\
&\resizebox{0.9\hsize}{!}{$M_{\mu\alpha\beta}\equiv \frac{1}{3}(2Q_{\mu\alpha\beta}-Q_{\alpha\beta\mu}-Q_{\beta\mu\alpha})-\frac{1}{9}(2Q_{1\mu} g_{\alpha\beta}-Q_{1\alpha} g_{\beta\mu}-Q_{1\beta} g_{\mu\alpha})+\frac{1}{9}(2Q_{2\mu} g_{\alpha\beta}-Q_{2\alpha} g_{\beta\mu}-Q_{2\beta} g_{\mu\alpha})$}.
\end{split}
\end{align}

After some algebra, we can see that \eqref{CondQEPS=Perlick} leads to a relation between vectorial and tensorial components of nonmetricity that reads
\begin{equation}\label{condEPSPerlick2}
\dot\ga^\mu\lr{S_{\mu\al\be}+M_{\mu\al\be}+\frac{1}{9}g_{\mu(\al}\lr{Q_{1\be)}-4Q_{2\be)}}}=0.
\end{equation}
Given the tracelessness of both $M$ and $S$ in any pair of indices, taking the trace of this equation in the two free indices, we find that 
\beq
\dot\ga^\mu\lr{Q_{1\mu}-4Q_{2\mu}}=0
\eeq
has to be satisfied if \eqref{condEPSPerlick2} is satisfied. This last equation is satisfied for every timelike path only if $Q_1=4Q_2$. Plugging this into the general equation \eqref{condEPSPerlick2}, we find that $M=-S$ should hold for it to be true for every timelike path. Thus $Q_1=4Q_2$ and $M=-S$ must be satisfied by the most general kind of nonmetricity satisfying that any EPS clock is a generalised clock. Plugging these conditions into \eqref{NMdecomposed} we see that a nonmetricity tensor satisfying these conditions is
\begin{equation}
Q=Q_2\otimes g=\frac{1}{4}Q_1\otimes g,
\end{equation}
namely, the most general kind of spacetime in which any EPS clock is a generalised clock and vice versa. In fact, a conclusion of the EPS paper is that from its construction based on the compatibility of the projective and conformal structures defined by freely falling massive and massless particles, one is led univocally to a Weyl geometry \cite{EPS}, though some subtleties have been  addressed in \cite{Trautman2012,Matveev:2013fpl,Scholz:2019tif,Matveev:2020wif}. That is the reason why the EPS time is irrevocably connected to the geometrical definition of time that uses the metric and the connection introduced by Perlick, and if one wants to develop a notion of proper time in a spacetime where free particles follow autoparallels of an affine connection with nontrivial nonmetricity, GPT can be a good candidate from the theoretical point of view, since it suitably generalises Riemannian and Perlick times\footnote{Though recall that, in general, one cannot find a variational principle for matter fields leading to them following the autoparallel curves of an arbitrary connection, it can be found for some particular connections.}. Without having much hopes that any real observer could be sensitive to this notion of time, but driven by pure curiousity, let us explore an important physical effect that such an observer would feel from the use of this geometrical time. Namely, what is known as the second clock effect. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{GPT and the second clock effect}\label{sec:SecondClock}

\begin{figure}
\centering
\includegraphics[scale=0.2]{Figures/Second_clock_tracks.pdf}
\caption{Synchronized clocks $c_{1}$ and $c_{2}$ follow world lines
$\gamma_{1}$ and $\gamma_{2}$, which are coincident from point $A$ to $B$,
where they are separated to follow the parts $\Gamma_{1}$ and $\Gamma_{2}$ of
these lines until point $C$, where they are once again joined and continue
together until point $D$.}%
\label{fig:fig1Clock}%
\end{figure}

As a postscript to the original paper by Weyl \cite{Weyl:1918ib}, in which he introduced his geometrisation of electromagnetism and gravitation by means of a Weyl-like nonmetricity tensor, Einstein criticised the proposal by stating that the theory would suffer from an unpleasant effect due to the nonintegrability of lengths, namely, the clock rate of the clocks in the theory would depend on their past histories, which would have imprints in \eg the spectral lines of atoms which have never been observed. This effect was later coined as the \textbf{second clock effect} \cite{brown2000}. In order to illustrate it, consider two clocks $c_{1}$ and $c_{2}$ synchronised at event $A$ as in figure \ref{fig:fig1Clock}, which are transported following the same curve until event $B$, then separated and transported along two different curves, $\Gamma_{1}$ and $\Gamma_{2}$, until event $C$, where they are rejoined and transported to event $D$ following the same curve again. The proper time $\tau_i$ measured by the clock number $i$ after going from event $C$ to event $D$ is given by 
\begin{align}\label{time1}
\tau_i =\frac{\dot\tau_i(u_{iC})}{\sqrt{g\lr{\dot\gamma_i(u_{iC}),\dot\gamma_i(u_{iC})}}}\int_{u_{iC}}^{u_{iD}}du \sqrt{g\lr{\dot\gamma_i(u),\dot\gamma_i(u)}} \;e^{-\frac{1}{2}\int_{u_{iC}}^u ds\frac{Q\lr{\dot\gamma_i(s),\dot\gamma_i(s),\dot\gamma_i(s)}}{g\lr{\dot\gamma_i(s),\dot\gamma_i(s)}}},
\end{align}
The times from $A$ to $C$ can be computed using Eq.(\ref{cond_add}) as
\begin{align}
&\tau_i(u_{iC})=\dot\tau_i(u_A)\sqrt{\frac{g\lr{\dot\gamma_i(u_{iC}),\dot\gamma_i(u_{iC})}}{g\lr{\dot\gamma_i(u_A),\dot\gamma_i(u_A)}}}e^{-\frac{1}{2}\int_{u_A}^{u_{iC}}ds\frac{Q\lr{\dot\gamma_i(s),\dot\gamma_i(s),\dot\gamma_i(s))}}{g\lr{\dot\gamma_i(s),\dot\gamma_i(s)}}}
\end{align}
where $u_i$ is the parameter of the generalised clock $\gamma_i$. As in \cite{Avalos:2016unj}, after a reparametrisation from $u_2$ to $u_1$, and using synchronisation at event $A$, namely $\dot\ga_1(u_A)=\dot\ga_2(u_A)$, $\dot\ga_1(u_{1C})=\dot\ga_2(u_{2C})=\dot\ga(u_C)$, from the above equations we find
\begin{align}
&{\tau}_2(u_D)=\tau(u_D)\frac{\dot\tau_2(u_A)}{\dot\tau(u_A)}e^{\frac{1}{2}\lrsq{\int_{u_A}^{u_{1C}}\frac{Q(\dot\gamma_1(s),\dot\gamma_1(s),\dot\gamma_1(s))}{g(\dot\gamma_1(s),\dot\gamma_1(s))}ds-\int_{u_A}^{{u}_{2C}} \frac{Q(\dot\gamma_2(s),\dot\gamma_2(s),\dot\gamma_2(s))}{g(\dot\gamma_2(s),\dot\gamma_2(s))}ds}}.
\end{align}
Since both clocks have the same scale at the event $A$, {\it i.e.}, ${\dot\tau}_1(u_A)=\dot\tau_2(u_A)$, we conclude that a clock that measures GPT will measure a second clock effect in presence of a general nonmetricity tensor given by
\beq\label{SecondClockEffect}
\bar{\tau}=\tau \exp\left[\frac{1}{2}\int_{\Gamma_1-\Gamma_2}\frac{Q\lr{\dot\gamma(s),\dot\gamma(s),\dot\gamma(s)}}{g\lr{\dot\gamma(s),\dot\gamma(s)}}ds\right].
\eeq
This expression reduces to the result found in \cite{Avalos:2016unj} in Weyl spacetimes. and it is invariant under the action of conformal transformations \eqref{conf-trans}, $\int_{\Gamma_1-\Gamma_2} d\phi=0$ ( $\Gamma_1-\Gamma_2$ is a closed path). Therefore our construction describes a conformally invariant second clock effect. The observability of this event depends on whether clocks sensitive to this notion of time can be built with the available matter content in the universe. In \cite{Delhom:2020vpe}, assuming that a muon proper time is the GPT\footnote{Yes, Iarley and me were still young and bold enough to assume that, and we were surprisingly allowed by our supervisors!} allowed us to set bounds on the irreducible components of the nonmetricity tensor background at the Muon Storage Ring of $|Q|\lesssim 10^{-14}cm$.

\section{Is it possible to build a clock that measures GPT?}

As a final discussion, let us quickly elaborate on the possibility of measuring this invariant notion of proper time. Namely, let us digress on the question of whether one can actually construct a generalised clock with the content of our universe, or whether it is just a funny theoretical concept. To that end, recall that a physical clock as a clock that measures time as experienced by physical observers, namely massive bodies. By means of a generalised M\"arkze-Wheeler construction, one could in principle build clocks by using light rays and autoparallels of the connection, instead of Riemannian ones, as done by M\"arkze and Wheeler in \cite{MarzkeWheeler,Desloge1989-DESATD}, and then study whether this construction bears any relation with GPT. Notice that if it is to be related with GPT, scale invariance should play a central role on this generalised M\"arkze-Wheeler construction. Nonetheless, even if the construction of generalised clocks is possible in this way, that does not guarantee that it is possible to find such clocks in nature. Particularly, one would need to find massive particles that follow autoparallel curves of an affine connection with nontrivial nonmetricity, thus implying a violation of the Einstein Equivalence Principle, which is strongly constrained experimentally \cite{Will:2014kxa}. Furthermore, as we discussed in  section \ref{sec:geodesics}, it is generally not possible to find an action principle for matter fields leading to autoparallel curves of an arbitrary connection as the ones followed by freely falling bodies\footnote{Though this is possible for some particular kinds of connections.}. 
 General relativity is constructed in such a way  that free test particles follow Riemannian geodesics due to the conservation of the energy-momentum tensor, which in turn is required by diffeomorphism invariance \cite{Geroch:1975uq}. In \ref{sec:geodesics}, we argued that the characteristic curves of the solutions to the field equations of minimally coupled fields do not follow autoparallel paths of a connection with nonmetricity, but rather Riemannian geodesics or autoparallels of a connection with some particular form of torsion in the case of minimally coupled fermions \cite{HEHL1971225,Rumpf:1979vh,Audretsch:1981xn,Nomura:1991yx,Cembranos:2018ipn}. Hence, they are not well suited to build generalised clocks within the M\"arkze-Wheeler construction. Particularly, unless muons are seen to couple nontrivially to the nonmetricity, were this a feature of our spacetime, they would not be measuring GPT. However, some proposals for different couplings have arisen recently. For instance, the case of integrable Weyl spacetimes was addressed in \cite{Romero:2012hs}, in which a coupling that obeys the gauge invariance of the geometry and makes free particles follow Weyl geodesics in this theory was proposed. This issue was also addressed in \cite{deCesare:2016mml} for non-integrable Weyl geometry, were the authors concluded that free particles should follow Riemannian geodesics. In the context of $f(Q)$-gravity, it has been recently proposed  \cite{Harko:2018gxr} a coupling with matter where an extra force arises in the equation describing propagation of freely falling particles when written as a Riemannian geodesic equation. More recently, the case of a non-minimal coupling between matter and geometry in manifolds endowed with a nonmetric connection has gained some attention \cite{Gomes:2018sbf,SanomiyaProceedings,Sanomiya:2020svg}. Thus, being optimistic, the issue of whether GPT can be regarded as physical might depend on the particular model, since the possibility of constructing a generalised clock within every model depends on its particular geometry-matter coupling. However, a case-by-case analysis is required to ascertain whether these clocks exist in each particular theory.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{4D Einstein-Gauss-Bonnet theory is not well defined}\label{sec:4DEGB}

In a recent work \cite{Glavan:2019inb} it was claimed that there exists a theory of gravitation in four spacetime dimensions which fulfils all the assumptions of the Lovelock theorem \cite{Lovelock:1972vz} yet not its conclusions. The authors formulated the usual Einstein-Gauss-Bonnet (EGB) theory in an arbitrary dimension $\dimM$ with a coupling constant for the Gauss-Bonnet term rescaled by a $1/(\dimM-4)$ factor, as defined by the following action
\begin{equation}\label{action}
    \cS=\int \mathrm{d}^{\dimM}x \sqrt{|-g|}\left[ \frac{{\mpl^2}}{2}R+\frac{\alpha}{\dimM-4}\mathcal{G}-\CosmC\right].
\end{equation}
Here $\Lambda_{0}$ is a cosmological constant term, $R$ is the (metric) Ricci scalar, and $\mathcal{G}$ the (metric) Gauss-Bonnet (GB) term. As it is well known, the GB term is a topological invariant only in $\dimM=4$, but not in higher dimensions, thus generally yielding a nontrivial contribution to the field equations in arbitrary $\dimM>4$. In \cite{Glavan:2019inb} it is claimed that the contribution of the Gauss-Bonnet (GB) term to the equations of motion is always proportional to a $(\dimM-4)$ factor, which in principle compensates the divergence introduced in the coupling constant, thus allowing for a well defined $\dimM\to4$ \textit{limit} at the level of the field equations. It was argued that a nontrivial correction to General Relativity due to the GB term in \eqref{action} remains in $\dimM=4$. The proposal in \cite{Glavan:2019inb} is now known as 4-dimensional Einstein-Gauss-Bonnet theory (4DEGB).

The above action is one of the celebrated Lovelock actions in arbitrary $\dimM$. In \cite{Glavan:2019inb} it is claimed that all the assumptions of Lovelock theorem hold for this action after the $D\rightarrow4$ prescription is enforced, though it was also claimed that the resulting field equations do violate the conclusions of the Lovelock theorem. This was supposed to be accomplished by defining a 4-dimensional diffeomorphism-invariant theory satisfying the metricity condition and having second-order field equations which differ from those of General Relativity (GR). The authors of \cite{Glavan:2019inb} then proceeded to show the consequences of these modifications to GR in some scenarios with a high degree of symmetry. These results gained an astonishing amount of attention shortly after publication, with many works studying the properties of the solutions presented in \cite{Glavan:2019inb}, and other works criticising several aspects of the 4DEGB proposal \cite{Bonifacio:2020vbk,Hennigar:2020lsl,Mahapatra:2020rds,Ai:2020peo,Gurses:2020ofy} while, in some cases, relating them to other well defined theories \cite{Lu:2020iav,Kobayashi:2020wqy,Tian:2020nzb,Fernandes:2020nbq,Shu:2020cjw}. In this chapter, we will present several arguments that debunk many of the claims in \cite{Glavan:2019inb}, relating our results to some of the above works.

Let us sum up some of the main ideas of the chapter. It was claimed in \cite{Glavan:2019inb} that the contribution of the GB term  to the field equations (and not just its trace) is proportional to $(\dimM-4)$, and that this would imply the GB contribution to the field equations vanishes in four spacetime dimensions. The authors of \cite{Glavan:2019inb} then consider a coupling constant with a $1/(\dimM-4)$ factor that would \textit{regularise} the otherwise vanishing GB contribution, now yield a finite correction to the four dimensional field equations. We will show that, besides a term proportional to $(\dimM-4)$, the GB term contributes to the field equations with an additional part from which no power of $(\dimM-4)$ can be factorized, but which nonetheless vanishes identically in $\dimM=4$. 

Regarding tensor perturbations in D4EGB we will reproduce the results of \cite{Glavan:2019inb} for linear perturbations around a maximally symmetric background. This allows to find that, at the linear level and around maximally symmetric backgrounds, the proposal only propagates a massless graviton and that the corrections to GR provided by the \textit{regularised} GB term only enter through a global $\alpha$-dependent factor multiplying the linear perturbation equations in GR. Nonetheless we will see that the field equations describing second-order perturbations contain ill-defined terms even around a Minkowskian background. Indeed, we will argue that unless one is considering solutions with enough symmetry so as to force a specific combination of Weyl tensors to vanish in arbitrary dimensions, the term that is not proportional to $(\dimM-4)$ in the field equations renders the full D4EGB field equations ill-defined.

Finally, we will comment on the geometries presented in \cite{Glavan:2019inb} as the $\dimM\to4$ \textit{limit} of the spherically symmetric solutions for EGB theory in $\dimM\geq5$ found in \cite{Boulware:1985wk}. We will see that the claim made in \cite{Glavan:2019inb} that no particle can reach the central curvature singularity in a finite proper time within these geometries does not hold for freely-falling trajectories with vanishing orbital angular momentum. Furthermore, we will show that the \textit{regularised} D4EGB field equations are not well defined in spherically symmetric spacetimes unless the contribution which is not proportional to $(\dimM-4)$ is artificially stripped away from the field equations. Also, in the case that this term is removed, we will see that the spherically symmetric geometries presented in \cite{Glavan:2019inb} are not solutions of the remaining field equations in $\dimM=4$.

\section{The $\dimM\to4$ prescription}\label{sec:Dto4}

Let us first comment on whether the $\dimM\to4$ prescription taken in \cite{Glavan:2019inb} corresponds to a well-defined continuous limiting process in a topological sense. To that end, consider the $k$-th order Lovelock term in an arbitrary dimension $\dimM$
\begin{align}
S^{(k)} 
& = \int \dfR^{a_1 a_2}\wedge...\wedge\dfR^{a_{2k-1} a_{2k}}\wedge \star (\fr_{a_1}\wedge...\wedge \fr_{a_{2k}}) 
 \label{eq: Lovelock general}
\end{align}
where Greek indices refer to a coordinate basis and Latin indices to a frame in which the metric is Minkowskian (see chapter \ref{sec:DifferentialGeometry}). If we analyse the problem in differential form notation, when varying the action with respect to the dual frame $\df^a$ we find
\begin{equation}\label{var1}
\star\frac{\delta S^{(k)}}{\delta \df^a} = (\dimM-2k)(\dimM-2k-1)!\ J^{(k)}_{ac}\ \df^c\,,
\end{equation}
where $J^{(k)}_{ac}$ is a regular tensor built from combinations of the Riemann tensor that differ for each $k$.
 
The second factor in the above equation comes from the contraction of two Levi-Civita symbols. Therefore, it is of combinatorial nature, namely, it essentially has to do with the counting of the number of possible antisymmetric permutations of a bunch of indices. Notice that this counting process is not a continuous process in which the number of indices being counted (or equivalently the dimension) can take any value, but it ought to be an integer one. Indeed, for \eqref{var1} to be valid, $\dimM$ must be greater than $2k$ because a $(-1)!$ cannot arise from counting possible permutations. Since \eqref{var1} is not valid for $\dimM=2k$, it cannot be stated that the factor $(\dimM-2k)$ is the responsible for the vanishing of \eqref{var1} in $\dimM=2k$. The reason under its vanishing can actually be traced back to the properties of $2k$-forms in $2k$ dimensions. Indeed, by explicitly writing the Hodge star operator\footnote{Recall section \ref{sec:MetricStructure}} in \eqref{eq: Lovelock general}, in the critical dimension we obtain
\begin{equation}
\star_g (\fr_{a_1}\wedge...\wedge \fr_{a_{2k}})\big|_{\scriptsize \dimM=2k} = F \varepsilon_{a_1 ... a_{2k}}\,,
\end{equation}
where $\varepsilon_{a_1 ... a_{2k}}$ is the Levi-Civita symbol, $F$ is a non-zero constant that depends on $k$. As a consequence of this, and the well-known fact that the curvature factors in the action do not contribute (via spin connection) to the dynamics in Lovelock theories \cite{Mardones:1990qc}, the equations of motion for the soldering forms are identically satisfied. Observe that this is no longer true if $\dimM>2k$, since, in that case, the Hodge dual of $\cofr_{a_1}\wedge...\wedge \cofr_{a_{2k}}$ is not a $0$-form and gives a nontrivial contribution to the equation of motion of the soldering form.

It is clarifying as well to consider \eqref{var1} as a metric variation, {\it i.e.} avoiding the differential form notation and working directly with the metric components. We can rewrite the general $k$-th order Lovelock term \eqref{eq: Lovelock general} in an arbitrary dimension $\dimM\geq 2k$ as\beq
\cS^{(k)}=\tfrac{(2k)!}{2^k}\int R_{\nu_1\nu_2}{}^{\mu_1 \mu_2}...R_{\nu_{2k-1}\nu_{2k}}{}^{\mu_{2k-1}\mu_{2k}} \delta_{\mu_1}^{[\nu_1}...\delta_{\mu_{2k}}^{\nu_{2k}]} \sqrt{|g|}\mathrm{d}^\dimM x \,, 
\eeq
and its variation with respect to the metric is not proportional to $(\dimM-4)$, but rather of the form
\begin{equation}
\frac{1}{\sqrt{|g|}}\frac{\delta S^{(k)}}{\delta g^{\mu\nu}} = (\dimM-2k) A_{\mu\nu} + W_{\mu\nu}, \label{eq: AW decomposition}
\end{equation}
where no $(\dimM-2k)$ factor can be extracted from $W_{\mu\nu}$. For instance, the first-order Lovelock term (the Einstein-Hilbert action) leads to $A^\text{EH}_{\mu\nu}=0$ and $W^\text{EH}_{\mu\nu}=G_{\mu\nu}$, which vanishes by algebraic reasons in $\dimM=2$. Analogously, by decomposing the Riemann tensor into its irreducible pieces (see {\it e.g.} \cite{Ortin:2004ms}), the second-order Lovelock term, {\it i.e.} the Gauss-Bonnet term, leads to\footnote{The calculations have been checked with \href{http://www.xact.es/}{xAct }. There is a Mathematica notebook in the supplementary material of \cite{Arrechea:2020evj} where the calculations are explicitly made.}
\begin{align}
&\resizebox{.9\textwidth}{!}{$A^\text{GB}_{\mu\nu}  =  \frac{\dimM-3}{(\dimM-2)^2} \Big[\frac{2\dimM}{\dimM-1}R_{\mu\nu} R -\frac{4(\dimM-2)}{\dimM-3}R^{\rho\lambda}C_{\mu\rho\nu\lambda}-4R_{\mu}{}^\rho R_{\nu\rho}+2g_{\mu\nu}R_{\rho\lambda}R^{\rho\lambda}-\frac{\dimM+2}{2(\dimM-1)}g_{\mu\nu} R^2 \Big]\,,$} \label{eq: Amn GaussBonnet}  \\
&W^\text{GB}_{\mu\nu} =  2 \left[ C_{\mu}{}^{\rho\lambda\sigma}C_{\nu\rho\lambda\sigma}-\frac{1}{4} g_{\mu\nu} C_{\tau\rho\lambda\sigma}C^{\tau\rho\lambda\sigma}\right] \,,
\end{align}
where we have introduced the Weyl tensor $C_{\mu\nu\rho\lambda}$. Taking this into account, the field equations arrived at from \eqref{action} in arbitrary dimension are\footnote{Since the trace of $W^\text{GB}_{\mu\nu}$ is proportional to $(\dimM-4)$, the divergence disappears from the trace of the equation of motion. This does not occur for the traceless piece of the equation.}
\begin{equation}\label{fieldeqs}
G_{\mu\nu}+\frac{1}{{\mpl^2}}\CosmC g_{\mu\nu}+\frac{2\alpha}{{\mpl^2}}\left(A^\text{GB}_{\mu\nu}+\frac{W^\text{GB}_{\mu\nu}}{\dimM-4}\right)=0\,.
\end{equation}
The \textit{regularization} prescription given in \cite{Glavan:2019inb} consisted on evaluating $\dimM=4$ after calculating the equations of motion in arbitrary $\dimM$. If this is done, while the $A^\text{GB}_{\mu\nu}$ term indeed provides a finite nontrivial correction to the Einstein field equations if the coupling constant of the GB term is $\alpha/(\dimM-4)$, the $W^\text{GB}_{\mu\nu}$ term will be ill-defined in this case since, in general, $W^\text{GB}_{\mu\nu}$ does not go to zero asymptotically as $(\dimM-4)$. Indeed, the reason for $W^\text{GB}_{\mu\nu}$ to vanish in $\dimM=4$ is that the Riemann tensor loses independent components as one lowers the dimension and, in $\dimM=4$, this loss of components imply that $W^\text{GB}_{\mu\nu}$ necessarily vanishes by algebraic reasons, analogously to what happens to the Einstein tensor in $\dimM=2$. In other words, the reason for these expressions to be zero in certain dimensions is that they are \textit{algebraic} identities fulfilled by the curvatures of all possible metrics in the critical dimension, as opposed to \textit{analytic} identities at which one could arrive by a continuous limiting process given a suitable topology. A somewhat simpler example of the fact that the vanishing of the GB variation is due to algebraic reasons is provided by Galileon or interacting massive vector field theories. There, it can be seen that due to the Cayley-Hamilton theorem, the interaction Lagrangian of a given order $k$ identically vanishes for dimensions higher than the critical dimension associated to $k$ \cite{BeltranJimenez:2016rff}. 

The authors of \cite{Glavan:2019inb} appeal to an analogy between their method and the method of dimensional regularisation commonly employed in quantum field theory. The dimensional regularization method allows to extract the divergent and finite contributions from integrals that are divergent in $\dimM=4$ but non-divergent for higher $\dimM$. It consists on considering the analytic continuation of such integrals to the complex plane as a function of the complexified dimension $\dimM$, and then taking the limit $\dimM\to 4$ in a manner that allows to separate the divergent and finite contributions of the integrals. A key aspect that ensures the well-definiteness of dimensional regularization as an analytic continuation is that the regularised integrals are scalar functions which have no algebraic structure sensitive to the number of dimensions of the space they are defined in.\footnote{Typically the tensorial structures within the integrals are extracted from them by employing Lorentz-covariance arguments, and therefore the integrals to regularise are scalar functions.} Note however that this is not the case for the Gauss-Bonnet term, which has a nontrivial tensorial structure that is not well defined for non-integer dimensions. Thus, although the process of dimensional regularization can be rigorously defined by using the smooth $\dimM\to4$ limit of the appropriate analytic continuation of the scalar integrals, this fails to be a continuous limiting process when the quantities involved have a nontrivial algebraic structure, such as tensors or $p$-forms do. It would also be interesting to attempt to find a precise mathematical meaning to the {\it limiting} procedure in the presence of tensor fields which satisfy certain algebraic identities only in a particular number of dimensions. This could be done, for instance, by introducing a formal limit (see {\it e.g.} \cite{Mazur:2001aa}) and studying its properties, though it looks like a highly nontrivial task.

\section{Perturbations around maximally symmetric backgrounds}\label{sec:maxsim}

Despite the above considerations note that, even though the {\it regularisation} method proposed in \cite{Glavan:2019inb} will not work in general, it suffices for finding solutions that satisfy enough symmetries so as to render the $W^\text{GB}_{\mu\nu}$ identically {zero} in arbitrary dimension. Thus, by symmetry-reducing the action before enforcing $\dimM=4$, we can get rid of the problematic $W^\text{GB}_{\mu\nu}$ term and arrive to well-defined equations of motion. This is the case, for instance, of all conformally flat geometries, which have an identically vanishing Weyl tensor in $D\geq4$, thus {satisfying} the desired property that $W^\text{GB}_{\mu\nu}=0$ in $\dimM\geq4$ which makes the $D\to4$ {\it limit} of the symmetry-reduced D4EGB field equations \eqref{fieldeqs} well defined. Maximally symmetric geometries, or FLRW spacetimes, are conformally flat, and therefore the $D\rightarrow4$ prescription yields well defined field equations in such cases. Let us analyse the maximally symmetric solutions of \eqref{fieldeqs} studied in \cite{Glavan:2019inb}. In these geometries, the Riemann tensor is given by
\begin{equation}\label{eq: max symm}
R_{\mu\nu}{}^{\rho\sigma}=\frac{\KMaxSym}{{\mpl^2}(\dimM-1)}\left(\delta^{\rho}_{\mu} \delta^{\sigma}_{\nu}-\delta^{\sigma}_{\mu} \delta^{\rho}_{\nu}\right),
\end{equation}
and $W^\text{GB}_{\mu\nu}$ vanishes in arbitrary dimensions as explained above. In this case, the variation of the GB term is indeed proportional to $(\dimM-4)$ and, therefore, after this symmetry-reduction of the action \eqref{action}, the field equations \eqref{fieldeqs} read
\begin{equation}\label{fieldeqssym}
   G_{\mu\nu}+\frac{1}{{\mpl^2}}\CosmC g_{\mu\nu}+\frac{2\alpha}{{\mpl^2}}A^\text{GB}_{\mu\nu}=0 \,,
\end{equation}\label{regularisedEOM}
where $A^\text{GB}_{\mu\nu}$ provides a regular,  $\alpha-$dependent correction to GR. Although these properties will be shared by all conformally flat solutions, we should bear in mind that arbitrary perturbations around these backgrounds will be sensitive to the ill-defined contributions that come from the $W^\text{GB}_{\mu\nu}$ dependence of the full D4EGB field equations \eqref{fieldeqs}. Remarkably, the ill-defined corrections which enter the equations of motion through the $\alpha W^\text{GB}_{\mu\nu}/(\dimM-4)$ term do not contribute to linear order in perturbation theory around a maximally symmetric background which, presumably, is the reason why these ill-defined contributions were not noticed in \cite{Glavan:2019inb}, where only linear perturbations were considered. Nonetheless, as we will see, the divergent terms related to $W^\text{GB}_{\mu\nu}$ will enter the perturbations at second-order. To show this, let us consider a general perturbation around a maximally symmetric background by splitting the full metric as
\begin{equation}
    g_{\mu\nu}=\bar{g}_{\mu\nu}+\epsilon h_{\mu\nu}
\end{equation}
where $\bar{g}_{\mu\nu}$ is a maximally symmetric solution of \eqref{fieldeqs}. Therefore, the left hand side of \eqref{fieldeqs} can be written as a perturbative series in $\epsilon$ of the form
\begin{equation}
     E^{(0)}{}_{\mu\nu}+\epsilon E^{(1)}{}_{\mu\nu}+\epsilon^2 E^{(2)}{}_{\mu\nu}+\ldots\,,
\end{equation}
where $E^{(0)}{}_{\mu\nu}=0$ are the background field equations, $E^{(1)}{}_{\mu\nu}=0$ are the equations for linear perturbations, and so on. Using the zeroth-order equation, the linear perturbations in $\dimM$ dimensions and around a maximally symmetric background are described by\footnote{Although \eqref{linearpert} and the equations for linear perturbations in \cite{Glavan:2019inb} differ by the ordering of the covariant derivatives of the $\nabla_{\rho}\nabla_{\nu}h^{\mu\rho}$ term and the sign in the mass term, our equation \eqref{fieldeqs} coincides with those in {\it e.g.} \cite{Ortin:2004ms} for linearized perturbations around a maximally symmetric background. In any case the difference is not physically relevant, as can be seen by choosing a particular gauge.}
\begin{align}
\resizebox{.87\textwidth}{!}{$\nabla^{\rho}\nabla^{\mu}h_{\nu\rho}+\nabla_{\rho}\nabla_{\nu}h^{\mu\rho}-\nabla^{\rho}\nabla_{\rho} h_{\mu\nu}-\nabla^{\mu}\nabla_{\nu}h  +\delta^{\mu}{}_{\nu}(\nabla^{\sigma}\nabla_{\sigma}h -\nabla_{\rho}\nabla_{\sigma}h^{\rho\sigma})-\frac{\KMaxSym}{{\mpl^2}} (\delta^\mu_\nu h-2h^\mu{}_\nu)=0\,,$}\label{linearpert}
\end{align}
where $h\equiv h^\sigma{}_\sigma$, the indices are risen and lowered with $\bar g^{\mu\nu}$, and the covariant derivatives are those associated to the Levi-Civita connection of the background metric $\bar{g}_{\mu\nu}$. By inspection, we can see that this equation is regular in $\dimM=4$. Furthermore, as noted in \cite{Glavan:2019inb}, the equation governing linear perturbations \eqref{linearpert} are those ocuring in GR when linearised around an arbitrary background. Let us now go to quadratic order in the perturbations. For our purpose it will be sufficient to consider perturbations around a Minkowskian background. By using the zeroth- and first-order perturbation equations, and enforcing a vanishing background curvature $\KMaxSym=0$, we can write the second-order perturbation equations $E^{(2)}{}_{\mu\nu}=0$ as (see the supplementary material of \cite{Arrechea:2020evj})
\begin{align}\label{quadraticpert}
\resizebox{.85\textwidth}{!}{$[\text{GR terms of }\mathcal{O}(h^{2})]_{\mu\nu} +\frac{\alpha}{{\mpl}^{2}(\dimM-4)} \times\Big\{
 -2\nabla_{\gamma}\nabla_{\alpha}h_{\nu\beta}\nabla^{\gamma}\nabla^{\beta}h_{\mu}{}^{\alpha}
 +2\nabla_{\gamma}\nabla_{\beta}h_{\nu\alpha}\nabla^{\gamma}\nabla^{\beta}h_{\mu}{}^{\alpha}$}\nonumber \\
\resizebox{.85\textwidth}{!}{$+2\nabla^{\gamma}\nabla^{\beta}h_{\nu}{}^{\alpha}\nabla_{\mu}\nabla_{\alpha}h_{\beta\gamma} 
 +2\nabla^{\gamma}\nabla^{\beta}h_{\mu}{}^{\alpha}\nabla_{\nu}\nabla_{\alpha}h_{\beta\gamma}-2\nabla^{\gamma}\nabla^{\beta}h_{\mu}{}^{\alpha}\nabla_{\nu}\nabla_{\beta}h_{\alpha\gamma} 
 -2\nabla^{\gamma}\nabla^{\beta}h_{\nu}{}^{\alpha}\nabla_{\mu}\nabla_{\beta}h_{\alpha\gamma}$}\nonumber \\
\resizebox{.85\textwidth}{!}{$-2\nabla_{\mu}\nabla^{\gamma}h^{\alpha\beta}\nabla_{\nu}\nabla_{\beta}h_{\alpha\gamma}
 +2\nabla_{\mu}\nabla^{\gamma}h^{\alpha\beta}\nabla_{\nu}\nabla_{\gamma}h_{\alpha\beta}+g_{\mu\nu}\big(
 2\nabla_{\delta}\nabla_{\beta}h_{\alpha\gamma}\nabla^{\delta}\nabla^{\gamma}h^{\alpha\beta}
 -\nabla_{\delta}\nabla_{\gamma}h_{\alpha\beta}\nabla^{\delta}\nabla^{\gamma}h^{\alpha\beta}$}\nonumber \\
  \qquad\qquad -\nabla_{\beta}\nabla_{\alpha}h_{\gamma\delta}\nabla^{\delta}\nabla^{\gamma}h^{\alpha\beta}\big) \Big\}=0 \,.
\end{align}

In view of the above expression,\footnote{Note that we have kept the covariant derivatives in \eqref{quadraticpert} since our result is not restricted to a particular coordinate choice.} it is apparent that even around a flat background, the $W^{\text{GB}}_{\mu\nu}$ piece of \eqref{fieldeqs} contributes to the second-order perturbation equations with a term that is ill-defined in $\dimM=4$. These findings provide a clear example which serves to show that the D4EGB field equations \eqref{fieldeqs} are generally ill-defined. As a remark, let us point out that our results are somewhat in the line to those found in \cite{Bonifacio:2020vbk}, where it was seen that the amplitudes of GB in the $\dimM\to4$ \textit{limit} correspond to those of a scalar-tensor theory where the scalar is infinitely strongly coupled. Hence, they concluded that this new pathological degree of freedom would only show up beyond linear order in perturbations.

Going beyond a Minkowskian background, perturbations around arbitrary maximally symmetric backgrounds \eqref{eq: max symm} pick up additional terms which diverge as $\Lambda/(\dimM-4)$ (see the supplementary material of \cite{Arrechea:2020evj}). Concretely, up to second-order in $h_{\mu\nu}$, there are $\mathcal{O}(\Lambda)$ terms of the form $h(\nabla^2 h)$ and $\mathcal{O}(\Lambda^2)$ terms of the form $h^2$. Consequently, $\Lambda$-proportional terms provide additional divergences which make de Sitter and anti-de Sitter backgrounds also ill-defined beyond linear order in perturbation theory.

\section{An action for the regularised equations?}\label{sec:action}

We have seen that, unless the $W^\text{GB}_{\mu\nu}$ term is stripped away from the field equations \eqref{fieldeqs} after taking the variation of the D4EGB action \eqref{action}, they will be, in general, ill-defined. Let us now comment on the possibility of finding a diffeomorphism-invariant action whose field equations in $\dimM\geq4$ yield the {\it stripped} equations, namely field equations of the form \eqref{fieldeqssym}.\footnote{Even though the $\dimM\to4$ process, if understood as a limit, will have the same conceptual problems described in section \ref{sec:Dto4}, in this case they might be swept under the rug since the $1/(\dimM-4)$ dependence actually disappears from the field equations.} To find such an action starting from the EGB one, we should be able to subtract a scalar from the EGB action so that the contribution $W^\text{GB}_{\mu\nu}$ disappears after taking the variation with respect to the metric, yet the diffeomorphism symmetry of the EGB action is not lost. In trying to find such a term, we are immediately led to an inconsistency due to the form of the Bianchi identities related to diffeomorphism invariance. To see this, note that the Bianchi identities associated to diffeomorphism-invariant actions imply that its variation with respect to the metric must be identically divergenceless  \cite{Ortin:2004ms}. Hence, given that the Gauss-Bonnet term, {\it i.e.} \eqref{eq: Lovelock general} with $k=2$, is diffeomorphism invariant, it must satisfy this identity. Hence, by using the A-W decomposition \eqref{eq: AW decomposition} and substituting $A^\text{GB}_{\mu\nu}$ with \eqref{eq: Amn GaussBonnet}, it follows that the off-shell relation
\begin{align}\label{DivW}
      \nabla^\mu W^\text{GB}_{\mu\nu} = - \frac{4(\dimM-4)}{\dimM-2}C_{\nu\rho\lambda\mu}\nabla^\mu R^{\rho\lambda}\,.
\end{align}
must be satisfied. Observe that the right-hand side of this equation is not identically zero in an arbitrary dimension, as can be seen by considering the following counterexample in five dimensions,
\begin{equation}
    {\textrm{d}}s^2={\textrm{d}}t^2 - {\textrm{e}}^{2t}{\textrm{d}}x^2- {\textrm{e}}^{4t}({\textrm{d}}y^2+{\textrm{d}}z^2+{\textrm{d}}w^2)\,,
\end{equation}
for which the equation \eqref{DivW} reads
\begin{equation}
    \nabla^\mu W^\text{GB}_{\mu\nu} = -4 \delta^t_\nu\neq0\,.
\end{equation}

Together with the fact that the variation with respect to the metric of any diffeomorphism-invariant action is identically divergence-free, the above result implies that the term $W^{\text{GB}}_{\mu\nu}$ does not come from an action that is a scalar under diffeomorphisms and built only with a metric. Consequently, there does not exist any term that can be added to the action \eqref{action} to cancel the $W^{\text{GB}}_{\mu\nu}$ contribution in the D4EGB field equations \eqref{fieldeqs} without spoiling its diffeomorphism-invariance. 
Other authors have proposed alternative ways to regularise the action \eqref{action}, generally leading to a scalar-tensor theory  of  the  Horndeski  family \cite{Lu:2020iav,Bonifacio:2020vbk,Fernandes:2020nbq,Hennigar:2020lsl},  thus leaving the Lovelock theorem intact.

We thus conclude that no diffeomorphism-invariant action can give the desired {\it stripped} field equations \eqref{fieldeqssym} in $\dimM\geq4$. Nevertheless, nothing prevents the existence of a non-diffeomorphism-invariant action having \eqref{fieldeqssym} as its field equations. Should it be possible to find such action, however, the absence of diffeomorphism invariance would potentially unleash the well known pathologies that occur in massive gravity (see {\it e.g.} \cite{Hinterbichler:2011tt,deRham:2014zqa}), thus propagating a Boulware-Deser ghost \cite{Boulware:1973my}. 

\section{Geodesic analysis of the spherically symmetric geometries}\label{sec:geodesic}

In addition to maximally symmetric and FLRW spacetimes, spherically symmetric geometries claimed to be solutions of D4EGB were also considered in \cite{Glavan:2019inb}, where it was stated that they are described by the 4-dimensional metric 
\begin{equation}\label{sphericallysymmetricmetric}
    {\textrm{d}}s^2 = A_{\pm}(r){\textrm{d}}t^2 -A_{\pm}^{-1}(r){\textrm{d}}r^2-r^2{\textrm{d}}\Omega^2_2\,,
\end{equation}
where $A_{\pm}(r)$ has the form
\begin{equation}\label{eq:metric}
A_{\pm}(r)=1+\frac{r^2}{32\pi\alpha G}\left[1\pm\sqrt{1+\frac{128\pi\alpha G^2 M}{r^3}}\right].
\end{equation}
First of all, let us point out that $\dimM-$dimensional spherically symmetric geometries described by metrics of the form \cite{Ortin:2004ms}
\begin{equation}\label{sphericalmetricD}
{\textrm{d}}s^2 = A(r){\textrm{d}}t^2 -A^{-1}(r){\textrm{d}}r^2-r^2{\textrm{d}}\Omega^2_{\dimM-2}\,,
\end{equation}
do not in general satisfy that $W^{\text{GB}}_{\mu\nu}=0$ in arbitrary $\dimM\geq4$. To see this, it suffices to restrict us to the 5-dimensional case, where there is a nontrivial condition for $W^{\text{GB}}_{\mu\nu}$ to vanish for metrics of the above form that reads
\begin{equation}
    r^2\frac{{\textrm{d}}^2A}{{\textrm{d}}r^2}-2r\frac{{\textrm{d}}A}{{\textrm{d}}r}+2A-2=0\,.
\end{equation}
This only happens for the particular case \mbox{$A=1+C_1 r+C_2 r^2$} where $C_i$ are integration constants. This suggests that \eqref{eq:metric} cannot be regarded as a solution of the D4EGB field equations, given that \eqref{fieldeqs} is not well-defined for $\dimM$-dimensional spherically symmetric metrics \eqref{sphericalmetricD} in the $\dimM\to4$ \textit{limit}. Indeed, as the authors of \cite{Glavan:2019inb} explain, the 4-dimensional spherically symmetric geometries  \eqref{eq:metric} were obtained by first re-scaling $\alpha$ with a $1/(\dimM-4)$ factor in the sherically symmetric solutions obtained in \cite{Boulware:1985wk} for EGB in $\dimM\geq5$, and then taking the $\dimM\to4$ \textit{limit} of these metrics, instead of solving the $\dimM\to4$ \textit{limit} of \eqref{fieldeqs}.

Nevertheless, it could be that the spherically symmetric geometries of \cite{Glavan:2019inb} are solutions of \eqref{fieldeqssym}, namely the {\it stripped}  field equation, after being stripped away of the pathological $W^{\text{GB}}_{\mu\nu}$ term. In the supplementary material of \cite{Arrechea:2020evj}, it can be seen that \eqref{fieldeqssym} has four different branches of solutions for $\alpha>0$. Two of them are exactly the Schwarzschild and Schwarzschild-(anti-)de Sitter
\begin{align}
    &A_1=1-\frac{2GM}{r}\,,\nonumber\\
    &A_2=1+\frac{r^{2}}{16\pi G \alpha}-\frac{2GM}{r}\,.
\end{align}
and the other two cannot be solved analytically, though their asymptotic behavior near the origin can be seen to be $A\cong r^{-3-2\sqrt{3}}+\mathcal{O}(r^0)$. Thus these solutions can neither be the ones found in \cite{Glavan:2019inb}, although they approach the Schwarzschild and Schwarzschild-(anti-)de Sitter solutions at spatial infinity.

Let us now turn to the behavior of the spherically symmetric geometries presented in \cite{Glavan:2019inb}. As noted in \cite{Glavan:2019inb}, the $\alpha<0$ branch of the above solution is not well defined {for values of the radial coordinate below $r<(-128\pi\alpha G^2 M)^{-1/3}$}, so their analysis focused on the $\alpha>0$ branches, showing that the above metric describes solutions which behave asymptotically as Schwarzschild or Schwarzschild-de Sitter solutions by choosing the negative and positive signs respectively. Concerning the former branch of solutions, it was shown in \cite{Glavan:2019inb} that {its} causal structure {(namely, the presence or absence of event horizons)} depends on the ratio between the {\it mass} {parameter} $M$ and a new mass scale $M_*=\sqrt{16\pi\alpha/G}$ that characterizes the D4EGB corrections to GR. From \eqref{sphericallysymmetricmetric} and \eqref{eq:metric} it can be shown that the $g_{tt}$ component of the metric {vanishes at the spherical surfaces}
\begin{equation}\label{eq:horizons}
    r_\pm=GM\left[1\pm\sqrt{1-\left(\frac{M_*}{M}\right)^2}\right].
\end{equation}
In view of this expression it becomes clear that solutions have no horizons for the $M<M_*$ case, outer and inner horizons if $M>M_*$ and one degenerate horizon if $M=M_*$. Interestingly, the mass scale $M_{*}$ plays a role similar to that of the electric (and magnetic) charges in the Reissner-Nordstr{\"o}m spacetime, with the exception that, in this case, the origin of such contributions comes exclusively from the gravitational field. The effect of the Gauss-Bonnet terms would then be that of making gravity repulsive at short distances, the magnitude of this repulsion being dictated by the strength of the GB coupling $\alpha$.

{Regarding the presence of singularities in the solutions, we see that despite the metric components \eqref{eq:metric} being finite at the origin} \begin{equation}
A(r)=1-\sqrt{\frac{2M}{GM_*^2}}r^{1/2}+\mathcal{O}(r^{3/2})\,,  
\end{equation}
curvature invariants diverge as $R\propto r^{-3/2}$, $R_{\mu\nu}R^{\mu\nu}\sim R_{\mu\nu\alpha\beta}R^{\mu\nu\alpha\beta}\propto r^{-3}$. {In \cite{Glavan:2019inb} it is argued that an observer could never reach this curvature singularity given the repulsive effect of gravity at short distances.} {This would imply} that the spacetime described by \eqref{sphericallysymmetricmetric} is complete in the sense that no (classical) physical observer ever reaches the curvature singularity at $r=0$ in a finite proper time. Nonetheless, there was no explicit proof in \cite{Glavan:2019inb} showing that this was indeed the case. We thus proceed to give a precise answer to the following question: does any (classical) physical observer reach the curvature singularity of \eqref{sphericallysymmetricmetric} in a finite proper time? To answer that question, it suffices to study the sub-class of radial and freely-falling (classical) observers, described by radial time-like geodesics. We will also consider radial null geodesics for illustrative purposes. 

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{Figures/timelike_revs.pdf}
    \caption{Plot of the radial ingoing trajectories (in units of $r_{\textrm{S}}=2M$) of a free-falling massive particle in the spacetime \eqref{sphericallysymmetricmetric} (dashed lines), and of the Schwarzschild solution (pastel colors) for different values of the $M$ parameter. At large distances trajectories are indistinguishable. We have chosen $M_{*}=G=1$, $r(0)=100~r_{\textrm{S}}$ and $E=1$ for visualisation purposes.}
    \label{IngoingGeodesics}
\end{figure}

 Consider the geodesic equation in the equatorial plane\footnote{Since spacetime is spherically symmetric, geodesics will lie in a plane, which can be chosen as the equatorial one in suitable coordinates. See {\it e.g.} \cite{Wald:1984rg} for details on the derivation of the geodesic equation and \cite{Olmo:2015bya} for the completeness analysis. } $\theta=\pi/2$ for the metric \eqref{sphericallysymmetricmetric},
\begin{equation}\label{geoeq}
\left(\frac{{\textrm{d}}r}{{\textrm{d}}\tau}\right)^2=E^2-V_{\text{eff}}(r), 
\end{equation}
with
\begin{equation}
V_{\text{eff}}(r)=A(r)\left(\frac{L^2}{r^2}-\kappa\right),
\end{equation}
and where $\tau$ is the proper time of the observer that moves along the solution $r(\tau)$. Here, $\kappa$ takes the values $\{-1,1,0\}$ for space-like, time-like and null geodesics respectively. $E$ and $L$ are constants of motion associated with time-translation and rotational symmetries respectively. It will suffice for our purpose to analyse radial geodesics, characterised by $L=0$. Firstly note that since radial photon trajectories are {insensitive} to the value of $A(r)$ in a spacetime described by any metric of the form \eqref{sphericallysymmetricmetric}, the trajectories stay the same as in GR. The solution to \eqref{geoeq} for time-like geodesics is plotted in Fig. \ref{IngoingGeodesics} for the cases with different causal structures. There, it can be seen that infalling massive particles starting in a region well beyond the Schwarzschild radius (where the space-time is effectively the same as in GR) reach the curvature singularity at $r=0$ in a finite proper time (no matter what its initial velocity is). Notice that, as can be seen in Fig. \ref{IngoingGeodesicsnear0}, the deviations from the GR trajectories are not relevant until the particle is at $r\cong r_{S}$. An asymptotic analysis of the geodesic equation reveals that, while in GR the curvature singularity at $r=0$ is reached with infinite velocity ${\textrm{d}}r/{\textrm{d}}\tau|_{\text{GR}}\propto r^{-1/2}+\mathcal{O}(r^{0})$, the geodesics described by \eqref{sphericallysymmetricmetric} reach it with finite velocity
\begin{equation}\label{eq:velocity}
  ({\textrm{d}}r/{\textrm{d}}\tau)^2|_{\text{D4EGB}}=E^{2}-1+\sqrt{2M/M_*^{2}}r^{1/2}+\mathcal{O}(r^{3/2})\,.
\end{equation}
It is interesting to note that in the case that the infalling particle starts at rest, no matter what its initial position is, it will reach the singularity with zero velocity (characterised by $E^2=1$): attractive and repulsive effects compensate each other along the trajectory of the particle.
\begin{figure}
    \centering
    \includegraphics[scale=0.7]{Figures/EGBGR_revs.pdf}
    \caption{Figure showing how the trajectories of a massive particle in the spacetime described by \eqref{sphericallysymmetricmetric} (in units of \mbox{$r_{\textrm{S}}=2M$}) deviate from those of the Schwarzschild solution from GR near the central curvature singularity. Here, the $M=0.5M_*$ case is shown, although all timelike geodesics show the same behavior near the singularity. Units are $M_{*}=G=1$.}
    \label{IngoingGeodesicsnear0}
\end{figure}
The above proves that the statement made in \cite{Glavan:2019inb} that particles cannot reach the central singularity in spacetimes described by \eqref{sphericallysymmetricmetric} do not stand a rigorous analysis, as the singularity is reached in finite affine parameter.  Therefore, the hope that these solutions avoid the singularity problem is cast into serious doubt. Furthermore, the authors of \cite{Glavan:2019inb} also claim that under a realistic stellar collapse, matter would stop before reaching the singularity. This of course must be verified by a self-consistent analysis of the dynamical collapsing geometry, as was done in \cite{Malafarina:2020pvl}, revealing that the singularity indeed forms and gets covered by a horizon. Furthermore, the authors of \cite{Malafarina:2020pvl} also found that if the collapse is modelled {\it \`a la} Oppenheimer-Snyder, where dust is initially at rest, matter reaches the singularity with zero velocity, in agreement with our results.

We also note that, even if geodesic observers did never arrive at the singularity, the usual problems regarding curvature singularities would still remain: quantum corrections would be expected to become non-perturbative near the singularity and the background could not be treated classically anymore. However, the solutions would be {\it classically} singularity free in this case.

\section*{Final remarks} 

Here we have looked upon the idea of providing corrections to four dimensional General Relativity by means of the Gauss-Bonnet term devised in \cite{Tomozawa:2011gp} and recently revisited in \cite{Glavan:2019inb}. We have shown that this idea cannot be implemented for the Gauss-Bonnet ($k$-th order Lovelock) term in four ($2k$) spacetime dimensions by means of the procedure considered in \cite{Glavan:2019inb} without encountering inconsistencies. When considering solutions with a high degree of symmetry, such as maximally symmetric or general conformally flat solutions, this issue gets concealed at the level of the equations of motion due to the fact that the problematic terms $W^\text{GB}_{\mu\nu}$ in \eqref{fieldeqs} vanish for arbitrary $\dimM$ in these scenarios. Indeed we have shown that, when considering perturbations around a Minkowskian (or any maximally symmetric) background beyond linear order, such inconsistencies are immediately unveiled. This is also aligned with the conclusions at which the authors of \cite{Bonifacio:2020vbk} arrived by analysing the tree-level graviton scattering amplitudes in a Lagrangian-independent way by taking the four dimensional limit of the corresponding scattering amplitudes in EGB in higher dimensions. 

Regarding the spherically symmetric geometries presented in \cite{Glavan:2019inb}, we showed that they do not attain the required degree of symmetry as to make the problematic $W^\text{GB}_{\mu\nu}$ term vanishing in arbitrary dimension and, thus, bypass the pathologies encountered in the D4EGB field equations \eqref{fieldeqs}. By artificially removing the divergent $W^\text{GB}_{\mu\nu}$ term from \eqref{fieldeqs}, we encountered four spherically symmetric solutions, none of which coincides with those presented in \cite{Glavan:2019inb}. We also showed that the corresponding {\it stripped} equations cannot be derived from a diffeomorphism covariant action built only with the metric. Moreover, a geodesic analysis of the geometries from \cite{Glavan:2019inb} contradicts the observation about the singularity being unreachable by any observer in finite proper time.

To conclude, let us point out that the idea of extracting nontrivial corrections to the dynamics of a theory from topological terms by considering a divergent coupling constant is indeed very appealing, since its range of applicability extends far beyond gravitational contexts. For instance, it might serve to introduce parity-violating effects in Yang-Mills theories through the corresponding $F\tilde F$ terms that are topological in four dimensions. Indeed, a similar idea has been seen to lead to well-defined theories in the context of Weyl geometry \cite{BeltranJimenez:2014iie,BeltranJimenez:2015pnp,BeltranJimenez:2016wxw}. It could thus be interesting to explore various possibilities in this direction.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%=========================================================
